Symbolic Path-guided Test Cases for Models with Data and Time

This paper focuses on generating test cases from timed symbolic transition systems. At the heart of the generation process are symbolic execution techniques on data and time. Test cases look like finite symbolic trees with verdicts on their leaves and are based on a user-specified finite symbolic path playing the role of a test purpose. Generated test cases handle data involved in time constraints and uninitialized parameters, leveraging the advantages of symbolic execution techniques.

==> 5_testcase-old.tex <==

%\subsection{Path-guided test case}
%\noindent {\bf Test case generation} 
Roughly speaking, a test case $\mathbb{TC}$ will be a mirror TIOSTS of a TIOSTS $\mathbb{G}$, restricted by $tp$, a test purpose of $\mathbb{G}$, intended to interact with a $LUT$ that we wish to check its conformance to $\mathbb{G}$ up to $tp$.
$\mathbb{TC}$ will be a tree-like TIOSTS with $tp$ of $\mathbb{G}$ as a backbone, incorporating the following specific characteristics:
%We will define a test case as a TIOSTS-like structure with a test purpose $tp$ as the backbone. More exactly, a test case will be a tree-like structure with the following particularities:
\begin{itemize}
    \item execution contexts in $\mathbb{EC}(tp)$ constitute the main branch,
    \item sink states or leaves are assimilated with a test verdict. Notably, the last execution context $tgt(tp)$ of $tp$ will be assimilated with the $\text{PASS}$ verdict,
    \item from each $ec$ in $\mathbb{EC}(tp)$ other than $tgt(tp)$, the outgoing arcs outside $tp$ decline all ways to deviate from $tp$ and directly lead to a verdict state, either an inconclusive verdict or a failure verdict.
    %\\ \commental{$\mathbb{EC}(tp)$ est requis (?) dans les règles !} \commentplg{J'ai mis dans les règles $(\mathbb{EC}(\mathbb{G}) \setminus  \mathbb{EC}(tp))$}
\end{itemize}    


In Def.\ref{def:test-case}, we define $\mathbb{TC}$ by enumerating the different cases of transitions to be built according to channel type and $tp$ membership. We now give a few indications for enhancing the definition readability. Channel roles are reversed: channels in $CC^{in}$ as well as %the particular
channel $\delta$ (resp. $C^{out} \cup UC^{in}$) become output (resp. input) channels. 
%Transitions from $tp$ on $CC^{in}$ are emission transitions in $\mathbb{TC}$, and symmetrically, transitions from $tp$ on $C^{out} \cup UC^{in}$ are receptions in $\mathbb{TC}$. 
Variables of $\mathbb{TC}$ will be 
 symbolic variables involved in $tp$ and will be used to store successive concrete events observed on $LUT$. Any observation  on $LUT$ will be encoded as an input transition in $\mathbb{TC}$, whether it is an emission from a channel of $C^{out}$, a reception on a channel of $UC^{in}$ or a time-out observation. On the latter, it is conventional to consider that a system that does not react before a certain delay, chosen to be long enough, is in a state of quiescence. The only notable exception is when input transitions of $tp$ give rise to output transitions for $\mathbb{TC}$, modeling a situation in which $\mathbb{TC}$ stimulates $LUT$ by sending it data. The choice of the data to send is conditioned by two constraints: (i) taking into account the information collected so far and stored in the variables of $\mathbb{TC}$ in the first steps, and (ii) the guarantee of being able to reach the last EC of $tp$, i.e. the verdict $\text{PASS}$. This will be done by ensuring the satisfiability of the path condition of $tp$, leaving aside the variables already binded. 
%The process of test case generation will be applied to the fully-prepared symbolic subtree containing ECs of the test purpose $tp$ denoted by $\mathbb{EC}(tp)$ and adjacent ECs $\mathbb{EC}_a(tp)$. The trace-deterministic property of $tp$ is verified for the execution contexts from this fully-prepared subtree as stated in Def~\ref{def:Test purpose} which is a perquisite to the following  test case definition.
% The process of test case generation will be applied to a fully-prepared symbolic subtree containing ECs of the test purpose $tp$ denoted by $\mathbb{EC}(tp)$ and adjacent ECs $\mathbb{EC}_a(tp)$. These are successors of the ECs composing $tp$ from which we exclude those of $tgt(tp)$, and any successor $ec$ with a controllable input,.i.e., $chan(ec)\in CC^{in}$ . Obviously, we also require $Sat(\pi(ec))$ for any $ec \in \mathbb{EC}_a(tp)$. As we restrict to trace-deterministic TIOSTS, we check Def.~\ref{def:Deterministic_TIOSTS} for execution contexts from this fully-prepared subtree.
%Finally, we consider a global maximal waiting-time denoted as a constant $\emph{TM}$, in order to bound the waiting delay for observing outputs or internal inputs emitted by other systems. The waiting-time fixed in the test case to avoid waiting for too long for such observations. For instance, it can be chosen as the maximal value among those which bound the occurrences of observations (outputs or uncontrollable inputs) in the definition of the test purpose.%, plus some duration.

We will refer to variables of a symbolic path as follows: for\footnote{For $i$ and $j$ in $\mathbb{N}$ verifying $i < j$, $[i,j)$ contains the integers from $i$ to $j-1$ included.} $\alpha \in \{in,out\}$, $f^\alpha(p)=\bigcup_{i \in [1,n)} f^\alpha(ec_i)$ will denote all introduced fresh variables in $F^\alpha$ used to compute a symbolic path $p =ec_0.ec_1\ldots ec_n$. Similarly, $f^{dur}(p) = \{ f^{dur}(ec_i) | i \in [1,n) \}$. Moreover, for a target execution context $ec_n = tgt(p)$, we denote $\overline{f}^\alpha(ec_n)$ and $\overline{f}(ec_n)$ resp. for $f^\alpha(p)$ and  $f(p)$. 

\begin{definition}[Path-guided test case]
\label{def:test-case}
Let $tp$ be a test purpose for a TIOSTS $\mathbb{G}$. 
Let us consider the signature $\widehat{\Sigma} = (\widehat{A}, \widehat{K}, \widehat{C})$ where: 
\begin{itemize}
    \item $\widehat{A} = f^{in}(tp) \cup f^{out}(tp)$, 
    \item $\widehat{K}=f^{dur}(tp)$, 
    \item $\widehat{C}=C_\delta$ such that $\widehat{C}^{in} = C^{out} \cup UC^{in}$ and $\widehat{C}^{out} = CC^{in} \cup \{\delta\}$
\end{itemize}    
A \emph{test case guided by} $tp$ is a TIOSTS $\mathbb{TC}=(\widehat{Q}, \widehat{q_0}, \widehat{Tr})$ over $\widehat{\Sigma}$ where: %where: $A_{\tc} = f^{in}(tp) \cup f^{out}(tp)$, $K_{\tc}=f^{dur}(tp)$, $C_{\tc}=C \cup \{\delta\}$ such that ${(C_{\tc})}^{in} = C^{out} \cup UC^{in}$ and ${(C_{\tc})}^{out} = CC^{in} \cup \{\delta\}$,  
\begin{itemize}
    \item $\widehat{Q} = \big(\mathbb{EC}(tp) \setminus \{tgt(tp)\} \big) \cup \mathbb{V}$ where: \\
    %~\footnote{Verdicts $\text{FAIL}^{out}$ and $\text{FAIL}^{dur}$ mean non-conformance w.r.t. tioco} 
    $\mathbb{V} = \{$
    $\emph{PASS},$
    $\emph{FAIL}^{out},$
    $\emph{FAIL}^{dur},$
    $\emph{INC}^{out},$
    $\emph{INC}^{dur},$
    % $\emph{INC}^{specUncI},$
    $\emph{INC}^\uncIn_\spec,$
    % $\emph{INC}^{unspecUncI}\},$
    $\emph{INC}^\uncIn_\unspec$
$\}$,
    \item $\widehat{q_0}=ec_0$,
    \item $\widehat{Tr}$ is defined by a set ${\cal R}$ of  10 rules of the form $(Ri)$ LABEL $\frac{H}{ tr\in  \widehat{Tr}}$ for $i \in [1,10]$. Such a rule reads as follows: the transition $tr$ can be added due to rule $Ri$ to $\widehat{Tr}$ provided that hypothesis $H$ holds and $Sat(tr)$.
\end{itemize}   

In writing the rules of ${\cal R}$, we will use the two formulas \\
\centerline{$\phi^\obs_\spec =
    (z < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))
$}
%$\phi^\obs_\spec$ 
\centerline{$\phi^\obs_\unspec =
        (f^{dur} (ec) < \emph{TM} ) \land  \bigwedge_{\substack{pec(ec') = ec \\ chan(ec')=c }}(\forall F^{ini}.\neg\pi(ec'))$} 
that occur several times in the rules
and the constant $\emph{TM}$ (Time-out) that limits the waiting-time for observing outputs or uncontrollable inputs. %The waiting-time fixed in the test case to avoid waiting for too long for such observations.
    


\vspace{.2cm}


{
\centering
\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.8}
\AxiomC{$
      ec \in \mathbb{EC}(tp)
\quad ev(ec) = (z, c?x)
\quad c \in CC^{in}
$}
\LeftLabel{
    (R1) \emph{SKIP}
%\stackanchor{{\bf R1 Stimulation}}{}
}
\UnaryInfC{
\stackanchor{ $\big(
      pec(ec)
\;,\; c!x
\;,\; \phi_{stim}
\;,\; \{ f^{dur} (ec) \}
\;,\; id_{\widehat{A}}
\;,\; ec \big) \in \widehat{Tr}$ }{$\phi_{stim} =
    (\exists F^{ini} \cup \overline{f}(tgt(tp)) %Var(\pi(tp))
    \setminus \overline{f}(ec). \pi(tp) )
$}
}
\end{scprooftree}
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.8}
\AxiomC{$
      ec \in \mathbb{EC}(tp)
\quad ev(ec)=(z, c!y)
\quad c \in C^{out}
\quad ec \neq tgt(tp)
$}
\LeftLabel{
    (R2) \emph{SKIP}
%\stackanchor{{\bf R2 Specified output}}{{\bf inside $tp$}}
}
\UnaryInfC{
$\big(      pec(ec)
\;,\; c?y
\;,\; \phi^\obs_\spec
\;,\; \{ f^{dur} (ec) \}
\;,\; id_{\widehat{A}}
\;,\; ec \big) \in \widehat{Tr}$ 
}
\end{scprooftree}
\end{minipage}

\vspace{.2cm}

\begin{minipage}{10cm}
\centering
\begin{scprooftree}{.8}
\AxiomC{
\stackanchor{$
      ec \in \mathbb{EC}(tp)
\quad ev(ec)=(z, c!y)
\quad c \in C^{out}
\quad ec = tgt(tp)
$}
{}
}
\LeftLabel{
    (R3) \emph{PASS}
% \stackanchor{
% {\bf R2 Specified output}}{{\bf inside $tp$ (last)}}
}
\UnaryInfC{
\stackanchor{$\big(
      pec(ec)
\;,\; c?y
\;,\; \phi^\obs_\spec
\;,\; \emptyset
\;,\; id_{\widehat{A}}
\;,\; \emph{PASS} \big) \in \widehat{Tr}
$}
{
% $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
}
}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.8}
\AxiomC{\stackanchor{$
%    ec \in (\mathbb{EC}(\mathbb{G}) \setminus  \mathbb{EC}(tp))
ec \in \mathbb{EC}(\mathbb{G})
\quad pec(ec) \in  \mathbb{EC}(tp) \setminus \{tgt(tp)\}
\quad ev(ec)=(z, c!y)
\quad c \in C^{out}
$}
{
% $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
}
}
\LeftLabel{
    (R4) $\emph{INC}^{out}$
%\stackanchor{{\bf R3 Specified output}}{{\bf outside $tp$}}
}
\UnaryInfC{$\big(
      pec(ec)
\;,\; c?y
\;,\; \phi^\obs_\spec
\;,\; \emptyset
\;,\; id_{\widehat{A}}
\;,\; \emph{INC}^{out}\big) \in \widehat{Tr}
$}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}


\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.8}
\AxiomC{\stackanchor{$
      ec \in \mathbb{EC}(tp)
\quad c \in C^{out}
$}
{}
}
\LeftLabel{
    (R5) $\emph{FAIL}^{out}$
%\stackanchor{{\bf R4 Unspecified output}}{{\bf}}
}
\UnaryInfC{
$\big(
      ec
\;,\; c?f^{out}_c(ec)
\;,\; \phi^\obs_\unspec
\;,\; \emptyset
\;,\; id_{\widehat{A}}
\;,\; \emph{FAIL}^{out}\big) \in \widehat{Tr}$}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.8}
\AxiomC{\stackanchor{$
      ec \in \mathbb{EC}(tp)
\quad ev(ec)=(z, c?x)
\quad c \in UC^{in}
$}
{}
}
\LeftLabel{
    (R6) \emph{SKIP}
%\stackanchor{{\bf R5 Specified uncontrollable}}{{\bf input inside $tp$}}
}
\UnaryInfC{
\stackanchor{$\big(
      pec(ec)
\;,\; c?x
\;,\; \phi^\obs_\spec
\;,\; \{ f^{dur} (ec) \}
\;,\; id_{\widehat{A}}
\;,\; ec \big) \in \widehat{Tr}$}{
%$\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
}
}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.8}
\AxiomC{
\stackanchor{$
      %ec \in (\mathbb{EC}(\mathbb{G}) \setminus  \mathbb{EC}(tp)) 
ec \in \mathbb{EC}(\mathbb{G})
\quad pec(ec) \in  \mathbb{EC}(tp) \setminus \{tgt(tp)\}
\quad ev(ec)=(z, c?x)
\quad c \in UC^{in}
$}
{}
}
\LeftLabel{
    % (R7) $\emph{INC}^{specUncI}$
    (R7) $\emph{INC}^\uncIn_\spec$
%\stackanchor{{\bf R6 Specified uncontrollable}}{{\bf input outside $tp$}}
}
\UnaryInfC{
\stackanchor{$\big(
      pec(ec)
\;,\; c?x
\;,\; \phi^\obs_\spec
\;,\; \emptyset
\;,\; id_{\widehat{A}} 
\;,\; \emph{INC}^\uncIn_\spec\big) \in \widehat{Tr}
$}
{
%$\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
}
}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.8}
\AxiomC{
\stackanchor{$
      ec \in \mathbb{EC}(tp)
\quad ev(ec)=(z, c?x)
\quad c \in UC^{in}
$}
{}
}
\LeftLabel{
    % (R8) $\emph{INC}^{unspecUncI}$
    (R8) $\emph{INC}^\uncIn_\unspec$
%\stackanchor{{\bf R7 Under-specified}}{{\bf uncontrollable input}}
}
\UnaryInfC{
\stackanchor{$\big(
      ec
\;,\; c?f^{in}_c(ec)
\;,\; \phi^\obs_\unspec
\;,\; \emptyset
\;,\; id_{\widehat{A}} 
\;,\; \emph{INC}^\uncIn_\unspec\big) \in \widehat{Tr}
$}
{
%$\phi^\obs_\unspec =  (f^{dur} (ec) < \emph{TM} ) \land  \bigwedge_{\substack{pec(ec') =ec \\ chan(ec')=c }}(\forall F^{ini}.\neg\pi(ec'))$
}
}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.8}
\AxiomC{
\stackanchor{
    $ec \in \mathbb{EC}(tp)$
}
{}
}
\LeftLabel{
    (R9) $\emph{INC}^{dur}$
%\stackanchor{{\bf R8 Specified quiescence}}{{\bf }}
}
\UnaryInfC{
\stackanchor{$\big(
      ec
\;,\; \delta!
\;,\; \phi^{\delta}_\spec
\;,\; \emptyset
\;,\; id_{\widehat{A}}
\;,\; \emph{INC}^{dur}\big) \in \widehat{Tr}
$}
{
$
    \phi^{\delta}_\spec = f^{dur}(ec) \geq \emph{TM}
    \land \bigvee_{\substack{pec(ec')=ec 
        \\ chan(ec') \in C^{out} \cup UC^{in} \cup \{\delta\}}} \exists F^{ini}.\pi(ec')
$
}}
\end{scprooftree}
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.8}
\AxiomC{\stackanchor{$ec \in \mathbb{EC}(tp)$}{}}
\LeftLabel{ (R10) $\emph{FAIL}^{dur}$
%\stackanchor{{\bf R9 Unspecified quiescence}}{{\bf }}
}
\UnaryInfC{
\stackanchor{$\big(
      ec , \delta!%\emph{TM}
\;,\; \phi^\delta_\unspec
\;,\; \emptyset
\;,\; id_{\widehat{A}} 
\;,\; \emph{FAIL}^{dur}\big)
    \in \widehat{Tr}
$}
{
$\phi^{\delta}_\unspec = f^{dur}(ec) \geq \emph{TM}
    \land \bigwedge_{\substack{pec(ec')=ec 
        \\ chan(ec') \in C^{out} \cup UC^{in} \cup \{\delta\}}} \forall F^{ini}.\neg \pi(ec')$
}}
\end{scprooftree}
\end{minipage}

% \begin{minipage}{11cm}
% \centering
% \begin{scprooftree}{.8}
% \AxiomC{\stackanchor{$ec \in \mathbb{EC}(tp)$}{}}
% \LeftLabel{ (R10) $\emph{FAIL}^{dur}$
% %\stackanchor{{\bf R9 Unspecified quiescence}}{{\bf }}
% }
% \UnaryInfC{
% \stackanchor{
% $\big(
%       ec
% \;,\; \delta!%\emph{TM}
% \;,\; \phi^\delta_\unspec
% \;,\; \emptyset
% \;,\; id_{A_{\emph{TC}}}
% \;,\; \emph{FAIL}^{dur}
% \big) \in Tr_{\tc}$}{
% \stackanchor{
%  $\phi^\delta_\unspec= f^{dur}(ec) \geq \emph{TM} \land
% \psi^\obs_\unspec$}
% {\stackanchor
% {$ \psi^\obs_\unspec=
%     \bigwedge{\substack{pec(ec')=ec \\ chan(ec') \in C^{out}}} \forall F^{ini}.\forall f^{out}_{chan(ec')}.\neg\pi(ec')
% $}
% {$ \land \bigwedge_{\substack{pec(ec')=ec \\ chan(ec') \in UC^{in}}} \forall F^{ini}. \forall f^{in}_{chan(ec')} . \neg \pi(ec')
% $}
% }
% }}
% \end{scprooftree}
% \end{minipage}
}
%\commental{La symétrie requise par mon biais cognitif ! :-)} \commentbb{Done + correction!}

% $\begin{array}{rllll}
%     \psi^\obs_\unspec =
%     &
%     \bigwedge{\substack{pec(ec')=ec \\ chan(ec') \in C^{out}}}
%     &
%     \forall F^{ini} .
%     &
%     \forall f^{out}_{chan(ec')} .
%     &
%     \neg\pi(ec')
% \\
%     \land
%     &
%     \bigwedge_{\substack{pec(ec')=ec \\ chan(ec') \in UC^{in}}}
%     &
%     \forall F^{ini}.
%     &
%     \forall f^{in}_{chan(ec')} .
%     &
%     \neg \pi(ec')
% \end{array}$

\end{definition}

%Generally speaking, 
A verdict $\text{PASS}$ is reached when $tp$ is covered, verdicts of the form $\text{INC}^m_n$ are reached when traces deviate from $tp$ while remaining in $\mathbb{G}$ and verdicts of the form $\text{FAIL}^m$ stand for traces outside $\mathbb{G}$. The annotations $n$ and $m$ provide additional information on the cause of the verdict. 
Rules $R1$, $R2$ and $R6$, grouped together under the label $\text{SKIP}$, allow advancing along $tp$, resp. by stimulating $LUT$ with the sending of data, observing an emission on $C^{out}$ and observing a reception on $UC^{in}$. Rule $R3$ (with the label $\text{PASS}$) indicates that the last EC of $tp$, thus the $\text{PASS}$ verdict, has been reached. Rules $R4$, $R7$, $R8$ and $R9$, each with a label of the form $\text{INC}^m_n$ indicate that the last observed event causes $LUT$ to leave $tp$, without however leaving $\mathbb{G}$, resp. by observing an output, an input specified in $\mathbb{G}$, an input not specified in $\mathbb{G}$ and a time-out observation. Lastly, rules $R5$ and $R10$, resp. labelled by  $\text{FAIL}^{out}$ and $\text{FAIL}^{dur}$, raise a $\text{FAIL}$ verdict, for resp. an unauthorized output and an exceeded time-out.

%We will comment more in details on the different rules and verdicts using Ex.~\ref{ex:test-case}. %Execution contexts of $tp$ become states of the test case except $tgt(tp)$ which is replaced by $\text{PASS}$. Every verdict state is connected to one or more contexts of $tp$:  Specified output, e.g., transition from $ec_2$ to $\text{INC}^{out}$ inferred from $ec_{10}$, specified uncontrollable input, e.g., transition from $ec_1$ to $\text{INC}^\uncIn_\spec$ inferred from $ec_9$, underspecified uncontrollable input ($\text{INC}^\uncIn_\unspec$), unspecified output ($\text{FAIL}^{out}$), and unspecified quiescence ($\text{FAIL}^{dur}$).



\begin{example}
\label{ex:test-case} In Fig.~\ref{fig:test_case_ATM}, the test case for $tp=ec_0ec_1\ldots ec_5$ (see Ex.~\ref{ex:tiosts-determ}) is depicted. Certain verdict states are repeated for readability, and defining rules annotate the transitions. The test case utilizes the $\text{Wdral}$ channel as a controllable input channel for stimulation while observing all other channels. For space considerations, we comment only on some rules.

 \noindent Rule $R1$ defines a stimulation action $\actOut{Wdral}\f{amt_1}$ (transition from $ec_1$ to $ec_2$) constrained by $\pi(tp)$ to select an appropriate value for $\f{amt_1}$ together with a time of stimulation $\f{z_1}$ that allows to remain within the test purpose. Within $\pi(tp)$, $\f{amt_1}$ is limited to the range $10\leq \f{amt_1} \leq 500$, while $\f{z_1}$ remains unconstrained (a duration measured with clock $\f{z_1}$, following the previous observation $\actIn{Init}$). It is worth noting that all non-revealed variables, i.e., other than $\f{z_0}$, $\f{z_1}$, and $\f{amt_1}$, appearing in $\pi(tp)$ are bound by the existential quantifier due to their unknown values at this stage of execution. Finally, the clock $\f{z_2}$ is reset to enable reasoning on subsequent actions' duration (measured on $\f{z_2}$).

\noindent  Rule $R2$ defines an observation action $\actIn{Debit}(\f{\freshOut{1}{D}{1}},\f{\freshOut{1}{D}{2}},\f{\freshOut{1}{D}{3}})$  constrained by 
$(\f{z_2}\!<\!\maxWaitingBound) 
\wedge \exists \f{fee_0} . \piAlias{3}$ (transition from $ec_2$ to $ec_3$) while rule $R5$ defines the same observation constrained by 
 $(\f{z_2}\!<\!\maxWaitingBound)
    \land \forall \f{fee_0} .
    \neg \, \piAlias{3}
    \land \forall \{ \f{fee_0} \} \, . \,
    \neg \, \piAlias{10}
    $ (transition from $ec_2$ to $\text{FAIL}^{out}$). Both situations are possible which shows from the following traces (the latter two diverge %from the test purpose
due to data resp. time non-compliance): 
    
    $(0,\actIn{Init}) .
    (0,\actOut{Wdral}50) .
    (0,\actIn{Debit}(1,51,\ATMID))$ reaches $ec_3$
    
    $(0,\actIn{Init}) . 
    (0,\actOut{Wdral}50) .
    (0,\actIn{Debit}(1,0,\ATMID)$ reaches $\text{FAIL}_{out}$ 
    
    $(0,\actIn{Init}) . 
    (0,\actOut{Wdral}50) .
    (2,\actIn{Debit}(1,51,\ATMID))$ reaches $\text{FAIL}_{out}$


\noindent Rule $R6$ defines an unspecified quiescence $\delta!$ constrained by $(\f{z_2} \geq \maxWaitingBound)
    \land %\big(
    \forall \f{fee_0} \, . \neg \piAlias{3}
    \land
    \forall \f{fee_0} \, . \neg \piAlias{10}
    \land
    \forall \f{fee_0} \, .\neg \piAlias{11}
    % \big)
$ (transition from $ec_2$ to $\text{FAIL}^{dur}$). This situation arises in the trace $(0,\actIn{Init}).(0,\actOut{Wdral}50).(5,\delta!)$, where time-out $\maxWaitingBound$ is set to $5$. In this case, the time-out is triggered without the mandatory output on the channel $\text{Debit}$ being observed. 

\noindent Rule $R9$ defines a specified quiescence $\delta!$ (transition from $ec_2$ to $\text{INC}^{dur}$ not drawn for space). This situation arises when there is still sufficient time to reach $ec_3$, $ec_{10}$ or $ec_{11}$ (n.b., no quiescence enrichment applies from $ec_2$, see Ex.~\ref{ex:quiescence}).
%for some trace $(0,\actIn{Init}).(0,\actOut{Wdral}50).(0,\delta!)$.
%\commentbb{SAY TEST CASE IS COMPLETE ON WHAT IT OBSERVES (OUT and UncINPUT)}
\end{example}
% that we cannot detail due to lack of space.

%\subsection{Soundness of test cases}
%In the meantime, will discuss how a test case can support test execution. %First, 
%Let us point out that by construction,  $\widehat{Q} \subseteq \mathbb{EC}(tp) \cup \mathbb{V}$ since the elements of $\mathbb{EC}(tp) \setminus \{ tgt(tp) \}$ are in %$\widehat{V}$
%$\widehat{Q}$ and the only other elements added are in $\mathbb{V}$, and thus are %leaves
%sink states of the test case $\mathbb{TC}$. So, the only states with a successor in $\mathbb{TC}$ are in $\mathbb{EC}(tp) \setminus \{ tgt(tp) \}$. 

\begin{figure}[t] %[h!]
    \centering
    %\makebox[.9\textwidth][c]{
    
    \resizebox{1\textwidth}{!}{
        \hspace{-1cm}\input{fig/tikz_atm_testcase_simplif}
    }
	\caption{Test case for $\text{ATM}$}
% Tentative version simplifiée pour la lisibilité.
	\label{fig:test_case_ATM}
 \vspace{-.5cm}
\end{figure}


We introduce an execution relation that will be helpful to abstract a synchronized execution of a trace with a test case: 
\begin{definition}[Relation execution $\leadsto_{\mathbb{TC}}$]
Let $\mathbb{G}$ be a TIOSTS and $tp$ a test purpose for $\mathbb{G}$ with $\mathbb{TC} = (\widehat{Q},\widehat{q_0},\widehat{Tr})$ the test case guided by $tp$.

The \emph{execution relation}  $\leadsto_{\mathbb{TC}}\subseteq \big( Evt(C_\delta)^* \times  \widehat{Q} \times M^F \big)^2$  is defined by:

for $ev.\sigma \in Evt(C_\delta)^*$, $q,q' \in \widehat{Q}$ and for $\nu, \nu' \in M^F$, $(ev.\sigma,q,\nu) ~\leadsto_{\mathbb{TC}}~ (\sigma, q',\nu')$ holds iff there exists $tr\in \widehat{Tr}$ s.t. $src(tr)\!=\! q$, $tgt(tr)\!=\!q'$, $\nu'(act(tr))=act(ev)$ and $M \models_{\nu'} \phi(tr)$ with $\nu'$ defined as:
 \begin{itemize}
     \item if $ev\!=\!(d,c?v)$ and $chan(tr)\!=\!c$ then $\nu'\!=\!\nu[f^{dur}(q)\!\mapsto\!d][ f^{in}_c(q)\!\mapsto\!v]$ ;
     \item if $ev\!=\!(d,c!v)$ and $chan(tr)\!=\!c$ then $\nu'\!=\!\nu[f^{dur}(q)\!\mapsto\!d][f^{out}_c(q) \!\mapsto\! v]$ :
     \item else, i.e., $ev\!=\!(d,\delta!)$ and $chan(tr)\!=\!\delta$, $\nu'=\nu[f^{dur}(q)\!\mapsto\!d]$.
 \end{itemize}
 \end{definition}


%Let $LUT$ a subset of $ Evt(C_\delta)^*$ satisfying ${\cal H}$. 
%We introduce an execution relation that abstracts a synchronized execution of a $LUT$, given as a subset of $Evt(C_\delta)^*$ satisfying ${\cal H}$, and the test case $\mathbb{TC}$: 
%\vspace{-.275cm}
%\[\leadsto_{\mathbb{TC}}\subseteq \big( Evt(C_\delta)^* \times  \widehat{Q} \times M^F \big)^2  \] 
%\vspace{-.575cm}

Intuitively, a step $(ev.\sigma, q,\nu) ~\leadsto_{\mathbb{TC}}~ (\sigma, q',\nu')$ consists in:
\begin{itemize}
    \item reading the first element $ev$ of a trace from a test case state $q$ and an interpretation $\nu$  synthesizing the known information about the variables in~$F$ \item building a new triple with $\sigma$ the trace remaining to be read, $q'$ a successor state of $q$ in $\widehat{Q}$, and $\nu'$ the updated interpretation of the variables~$F$. 
\end{itemize}

Let $LUT$ be a subset of $ Evt(C_\delta)^*$ satisfying ${\cal H}$ and $\overset{*}{\leadsto}_{\mathbb{TC}}$ be the reflexive and transitive closure of  $\leadsto_{\mathbb{TC}}$. Given a $LUT$ trace $\sigma_0$, we apply the execution relation iteratively from an initial triplet consisting of $\sigma_0$, $ec_0$ an initial EC and $\nu_0$ an arbitrary interpretation, to obtain the corresponding test verdict for $tp$, so that the verdict set obtained from the execution of $\mathbb{TC}$ on $LUT$ is defined by: 

%\noindent $vdt(LUT,\mathbb{TC})= \bigcup_{\substack{\sigma_0\in LUT ,\; \nu_0 \in M^F \\ \text{V}\in\mathbb{V}}}\{\text{V} ~|~ (\sigma_0,{q_0}_{\tc}, \nu_0) \overset{*}{\leadsto}_{\mathbb{TC}} (\sigma,\text{V}, \nu )\}$. 

\noindent $vdt(LUT,\mathbb{TC})= \{\text{V} ~|~ \exists \sigma_0 \in LUT, \nu_0 \in M^F, \text{V} \in \mathbb{V}, (\sigma_0,{q_0}_{\tc}, \nu_0) ~\overset{*}{\leadsto}_{\mathbb{TC}} (\sigma,\text{V}, \nu )\}$. 

\noindent Th.~\ref{th:corr} states the soundness of test case execution (see proof in Appendix~\ref{anx:proof}).

\begin{theorem}
\label{th:corr} 
Let $C$ be a set of channels. Let $\mathbb{G}$ and $LUT$ be resp. a TIOSTS defined on $C$ and a subset of $Evt(C_\delta)^*$ satisfying $\cal{H}$. \\
 If $LUT~tioco~\mathbb{G}$ then for any test purpose $tp$ for $\mathbb{G}$ with $\mathbb{TC}$ as test case guided by $tp$, we have $\emph{FAIL}^{out}\not\in vdt(LUT, \mathbb{TC}) $ and $\emph{FAIL}^{dur}\not\in vdt(LUT, \mathbb{TC})$.
\end{theorem}

 

Our test cases can be executed by designing a test program that maintains the following elements: (1) a current state of the test case, some execution context $ec$ (unique by trace-determinism), which is updated by following a test case transition $tr$ corresponding to applied stimulations or processed observations, and (2) a current interpretation $\nu$ that is significant for the revealed variables so-far (from the set $\overline{f}(ec)$). The interpretation $\nu$ is used to evaluate transition guards (whether $M \models_\nu \phi(tr)$) to determine the stimulation's value and the time to send the value or to check observation's value and occurrence time. The test program terminates when a verdict state of the test case is reached. 

{\em Implementation issues.} The test case generation is implemented as module in the Diversity symbolic execution platform~\cite{diversity}. Resulting test cases are expressed in Diversity's entry language, allowing their exploration through symbolic execution with the SMT-solver Z3~\cite{Z3}. 
%to verify the reachability of divergent transitions. 
%We minimize the test cases by keeping only reachable transitions. 
For easier execution, we export the test cases from Diversity in JSON format, with transition guards expressed in the SMT-LIB input format for SMT-solvers. We applied the test case generation module to the ATM example on an Intel Core i7. Throughout the experiment, we varied the size of the test purposes, measured in transitions of the reference TIOSTS, ranging from $5$ (discussed in Ex.~\ref{ex:test-case}) to $10$, \ldots, $100$. Our module successfully verified trace-determinism for all test purposes. However, we noticed a significant increase in generation duration as the test purpose size increased, while still remaining practicable. Specifically, generating the TIOSTS test case ($513$ transitions) for the test purpose of $100$ transitions took more than $40$s, in contrast to only $500$ms for the test purpose of size $5$ ($31$ transitions) resp. $8$s for the test purpose of size $50$ ($138$ transitions).


%A simple way of executing our test cases is to design a test program which maintains {\bf{\em (1)}} a current state issued from the test case, i.e., some execution context $ec$ (unique by trace-determinism), which is updated by following some test case transition $tr$ corresponding to a stimulation it applies or an available observation it processes, and {\bf{\em (2)}} a current interpretation $\nu$ significant for the revealed variables so-far, those from the set $\overline{f}(ec)$ that is used to assess transitions' guards (whether $\nu \models \phi(tr)$). The transitions' guards are used to compute stimulations and their submission time (obtained by solving $\phi(tr)$ and remembered through $\nu$) %(proposed by the solver) or to verify observations and their occurrence time (matched through $\nu$ that is checked to satisfy $\phi(tr)$). The test program terminates whenever a verdict state of the test case is reached. We have implemented our test case generation as a module of the symbolic execution platform Diversity~\cite{diversity}.
%A generated test case is expressed in Diversity's entry language as for the reference TIOSTS which allows its exploration by symbolic execution coupled with SMT-solver Z3~\cite{Z3}, e.g., to check the reachability of divergent transitions. We reduce (minimize) the test case to only those reachable transitions. To ease test cases execution, we have exported them from Diversity in the JSON format where test case transitions' guards are expressed in the input format for SMT-solvers, called SMT-LIB.

%We have implemented our test case generation as a module of the symbolic execution platform Diversity~\cite{diversity}. A generated test case is expressed in Diversity xLIA modeling language as for the reference TIOSTS. The test case can then be animated by symbolic execution in Diversity, e.g., to verify the reachability of divergent transitions. Constraint solving required in symbolic execution is done thanks to the SMT-solver Z3~\cite{}. If some divergent transitions are not reachable, we remove them from the test case and reduce (minimize) it to only those reachable transitions. To ease test execution, we have exported it from Diversity in the JSON format where the test case transitions' guards are expressed in the input format for SMT-solvers, called SMT-LIB.










==> 5_testcase-old1.tex <==

%\subsection{Path-guided test case}
%\noindent {\bf Test case generation} 
Roughly speaking, a test case $\mathbb{TC}$ will be a mirror TIOSTS of a TIOSTS $\mathbb{G}$, restricted by $tp$, a test purpose of $\mathbb{G}$, intended to interact with a $LUT$ that we wish to check its conformance to $\mathbb{G}$ up to $tp$.
$\mathbb{TC}$ will be a tree-like TIOSTS with $tp$ of $\mathbb{G}$ as a backbone, incorporating the following specific characteristics:
%We will define a test case as a TIOSTS-like structure with a test purpose $tp$ as the backbone. More exactly, a test case will be a tree-like structure with the following particularities:
\begin{itemize}
    \item execution contexts in $\mathbb{EC}(tp)$ constitute the main branch,
    \item sink states or leaves are assimilated with a test verdict. Notably, the last execution context $tgt(tp)$ of $tp$ will be assimilated with the $\text{PASS}$ verdict,
    \item from each $ec$ in $\mathbb{EC}(tp)$ other than $tgt(tp)$, the outgoing arcs outside $tp$ decline all ways to deviate from $tp$ and directly lead to a verdict state, either an inconclusive verdict or a failure verdict.
    %\\ \commental{$\mathbb{EC}(tp)$ est requis (?) dans les règles !} \commentplg{J'ai mis dans les règles $(\mathbb{EC}(\mathbb{G}) \setminus  \mathbb{EC}(tp))$}
\end{itemize}    


In Def.\ref{def:test-case}, we define $\mathbb{TC}$ by enumerating the different cases of transitions to be built according to channel type and $tp$ membership. We now give a few indications for enhancing the definition readability. Channel roles are reversed: channels in $CC^{in}$ as well as %the particular
channel $\delta$ (resp. $C^{out} \cup UC^{in}$) become output (resp. input) channels. 
%Transitions from $tp$ on $CC^{in}$ are emission transitions in $\mathbb{TC}$, and symmetrically, transitions from $tp$ on $C^{out} \cup UC^{in}$ are receptions in $\mathbb{TC}$. 
Variables of $\mathbb{TC}$ will be 
 symbolic variables involved in $tp$ and will be used to store successive concrete events observed on $LUT$. Any observation  on $LUT$ will be encoded as an input transition in $\mathbb{TC}$, whether it is an emission from a channel of $C^{out}$, a reception on a channel of $UC^{in}$ or a time-out observation. On the latter, it is conventional to consider that a system that does not react before a certain delay, chosen to be long enough, is in a state of quiescence. The only notable exception is when input transitions of $tp$ give rise to output transitions for $\mathbb{TC}$, modeling a situation in which $\mathbb{TC}$ stimulates $LUT$ by sending it data. The choice of the data to send is conditioned by two constraints: (i) taking into account the information collected so far and stored in the variables of $\mathbb{TC}$ in the first steps, and (ii) the guarantee of being able to reach the last EC of $tp$, i.e. the verdict $\text{PASS}$. This will be done by ensuring the satisfiability of the path condition of $tp$, leaving aside the variables already binded. 
%The process of test case generation will be applied to the fully-prepared symbolic subtree containing ECs of the test purpose $tp$ denoted by $\mathbb{EC}(tp)$ and adjacent ECs $\mathbb{EC}_a(tp)$. The trace-deterministic property of $tp$ is verified for the execution contexts from this fully-prepared subtree as stated in Def~\ref{def:Test purpose} which is a perquisite to the following  test case definition.
% The process of test case generation will be applied to a fully-prepared symbolic subtree containing ECs of the test purpose $tp$ denoted by $\mathbb{EC}(tp)$ and adjacent ECs $\mathbb{EC}_a(tp)$. These are successors of the ECs composing $tp$ from which we exclude those of $tgt(tp)$, and any successor $ec$ with a controllable input,.i.e., $chan(ec)\in CC^{in}$ . Obviously, we also require $Sat(\pi(ec))$ for any $ec \in \mathbb{EC}_a(tp)$. As we restrict to trace-deterministic TIOSTS, we check Def.~\ref{def:Deterministic_TIOSTS} for execution contexts from this fully-prepared subtree.
%Finally, we consider a global maximal waiting-time denoted as a constant $\emph{TM}$, in order to bound the waiting delay for observing outputs or internal inputs emitted by other systems. The waiting-time fixed in the test case to avoid waiting for too long for such observations. For instance, it can be chosen as the maximal value among those which bound the occurrences of observations (outputs or uncontrollable inputs) in the definition of the test purpose.%, plus some duration.

We will refer to variables of a symbolic path as follows: for\footnote{For $i$ and $j$ in $\mathbb{N}$ verifying $i < j$, $[i,j)$ contains the integers from $i$ to $j-1$ included.} $\alpha \in \{in,out\}$, $f^\alpha(p)=\bigcup_{i \in [1,n)} f^\alpha(ec_i)$ will denote all introduced fresh variables in $F^\alpha$ used to compute a symbolic path $p =ec_0.ec_1\ldots ec_n$. Similarly, $f^{dur}(p) = \{ f^{dur}(ec_i) | i \in [1,n) \}$. Moreover, for a target execution context $ec_n = tgt(p)$, we denote $\overline{f}^\alpha(ec_n)$ and $\overline{f}(ec_n)$ resp. for $f^\alpha(p)$ and  $f(p)$. 

\begin{definition}[Path-guided test case]
\label{def:test-case}
Let $tp$ be a test purpose for a TIOSTS $\mathbb{G}$. 
Let us consider the signature $\widehat{\Sigma} = (\widehat{A}, \widehat{K}, \widehat{C})$ where: 
\begin{itemize}
    \item $\widehat{A} = f^{in}(tp) \cup f^{out}(tp)$, 
    \item $\widehat{K}=f^{dur}(tp)$, 
    \item $\widehat{C}=C_\delta$ such that $\widehat{C}^{in} = C^{out} \cup UC^{in}$ and $\widehat{C}^{out} = CC^{in} \cup \{\delta\}$
\end{itemize}    
A \emph{test case guided by} $tp$ is a TIOSTS $\mathbb{TC}=(\widehat{Q}, \widehat{q_0}, \widehat{Tr})$ over $\widehat{\Sigma}$ where: %where: $A_{\tc} = f^{in}(tp) \cup f^{out}(tp)$, $K_{\tc}=f^{dur}(tp)$, $C_{\tc}=C \cup \{\delta\}$ such that ${(C_{\tc})}^{in} = C^{out} \cup UC^{in}$ and ${(C_{\tc})}^{out} = CC^{in} \cup \{\delta\}$,  
\begin{itemize}
    \item $\widehat{Q} = \big(\mathbb{EC}(tp) \setminus \{tgt(tp)\} \big) \cup \mathbb{V}$ where: \\
    %~\footnote{Verdicts $\text{FAIL}^{out}$ and $\text{FAIL}^{dur}$ mean non-conformance w.r.t. tioco} 
    $\mathbb{V} = \{$
    $\emph{PASS},$
    $\emph{FAIL}^{out},$
    $\emph{FAIL}^{dur},$
    $\emph{INC}^{out},$
    $\emph{INC}^{dur},$
    % $\emph{INC}^{specUncI},$
    $\emph{INC}^\uncIn_\spec,$
    % $\emph{INC}^{unspecUncI}\},$
    $\emph{INC}^\uncIn_\unspec$
$\}$,
    \item $\widehat{q_0}=ec_0$,
    \item $\widehat{Tr}$ is defined by a set ${\cal R}$ of  10 rules of the form $(Ri)$ LABEL $\frac{H}{ tr\in  \widehat{Tr}}$ for $i \in [1,10]$. Such a rule reads as follows: the transition $tr$ can be added due to rule $Ri$ to $\widehat{Tr}$ provided that hypothesis $H$ holds and $Sat(tr)$.
\end{itemize}   

In writing the rules of ${\cal R}$, we will use the two formulas \\
\centerline{$\phi^\obs_\spec =
    (z < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec'))
$}
%$\phi^\obs_\spec$ 
\centerline{$\phi^\obs_\unspec =
        (f^{dur} (ec) < \emph{TM} ) \land  \bigwedge_{\substack{pec(ec') = ec \\ chan(ec')=c }}(\forall F^{ini}.\neg\pi(ec'))$} 
that occur several times in the rules
and the constant $\emph{TM}$ (Time-out) that limits the waiting-time for observing outputs or uncontrollable inputs. %The waiting-time fixed in the test case to avoid waiting for too long for such observations.
    


\vspace{.2cm}


{
\centering
\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.75}
\AxiomC{$
      ec,ec' \in \mathbb{EC}(tp)
\quad pec(ec')=ec \quad ev(ec') = (z, c?x)
\quad c \in CC^{in}
$}
\LeftLabel{
    (R1) \emph{SKIP}
%\stackanchor{{\bf R1 Stimulation}}{}
}
\UnaryInfC{
\stackanchor{ $\big(
      ec
\;,\; c!x
\;,\; \phi_{stim}
\;,\; \{ f^{dur} (ec) \}
\;,\; id_{\widehat{A}}
\;,\; ec'
\big) \in \widehat{Tr}$ }{$\phi_{stim} =
    (\exists F^{ini} \cup \overline{f}(tgt(tp)) %Var(\pi(tp))
    \setminus \overline{f}(ec'). \pi(tp) )
$}
}
\end{scprooftree}
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.75}
\AxiomC{$
      ec,ec' \in \mathbb{EC}(tp)
\quad pec(ec')=ec
\quad ev(ec')=(z, c!y)
\quad c \in C^{out}
\quad ec' \neq tgt(tp)
$}
\LeftLabel{
    (R2) \emph{SKIP}
%\stackanchor{{\bf R2 Specified output}}{{\bf inside $tp$}}
}
\UnaryInfC{
$\big( ec
\;,\; c?y
\;,\; \phi^\obs_\spec
\;,\; \{ f^{dur} (ec') \}
\;,\; id_{\widehat{A}}
\;,\; ec' \big) \in \widehat{Tr}$ 
}
\end{scprooftree}
\end{minipage}

\vspace{.2cm}

\begin{minipage}{10cm}
\centering
\begin{scprooftree}{.75}
\AxiomC{
\stackanchor{$
      ec,ec' \in \mathbb{EC}(tp)
\quad pec(ec')=ec
\quad ev(ec')=(z, c!y)
\quad c \in C^{out}
\quad ec' = tgt(tp)
$}
{}
}
\LeftLabel{
    (R3) \emph{PASS}
% \stackanchor{
% {\bf R2 Specified output}}{{\bf inside $tp$ (last)}}
}
\UnaryInfC{
\stackanchor{$\big(
     ec
\;,\; c?y
\;,\; \phi^\obs_\spec
\;,\; \emptyset
\;,\; id_{\widehat{A}}
\;,\; \emph{PASS} \big) \in \widehat{Tr}
$}
{
% $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
}
}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.75}
\AxiomC{\stackanchor{$
%    ec \in (\mathbb{EC}(\mathbb{G}) \setminus  \mathbb{EC}(tp))
ec \in  \mathbb{EC}(tp) \setminus \{tgt(tp)\} \quad ec' \in \mathbb{EC}(\mathbb{G})
\quad pec(ec')=ec
\quad ev(ec')=(z, c!y)
\quad c \in C^{out}
$}
{
% $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
}
}
\LeftLabel{
    (R4) $\emph{INC}^{out}$
%\stackanchor{{\bf R3 Specified output}}{{\bf outside $tp$}}
}
\UnaryInfC{$\big(
      ec
\;,\; c?y
\;,\; \phi^\obs_\spec
\;,\; \emptyset
\;,\; id_{\widehat{A}}
\;,\; \emph{INC}^{out}\big) \in \widehat{Tr}
$}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}


\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.75}
\AxiomC{\stackanchor{$
      ec \in \mathbb{EC}(tp)
\quad c \in C^{out}
$}
{}
}
\LeftLabel{
    (R5) $\emph{FAIL}^{out}$
%\stackanchor{{\bf R4 Unspecified output}}{{\bf}}
}
\UnaryInfC{
$\big(
      ec
\;,\; c?f^{out}_c(ec)
\;,\; \phi^\obs_\unspec
\;,\; \emptyset
\;,\; id_{\widehat{A}}
\;,\; \emph{FAIL}^{out}\big) \in \widehat{Tr}$}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.75}
\AxiomC{\stackanchor{$
      ec,ec' \in \mathbb{EC}(tp)
\quad pec(ec') = ec
\quad ev(ec')=(z, c?x)
\quad c \in UC^{in}
$}
{}
}
\LeftLabel{
    (R6) \emph{SKIP}
%\stackanchor{{\bf R5 Specified uncontrollable}}{{\bf input inside $tp$}}
}
\UnaryInfC{
\stackanchor{$\big(
      ec
\;,\; c?x
\;,\; \phi^\obs_\spec
\;,\; \{ f^{dur} (ec') \}
\;,\; id_{\widehat{A}}
\;,\; ec' \big) \in \widehat{Tr}$}{
%$\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
}
}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.75}
\AxiomC{
\stackanchor{$
ec \in  \mathbb{EC}(tp) \setminus \{tgt(tp)\}
\quad
ec' \in \mathbb{EC}(\mathbb{G})
\quad pec(ec')=ec
\quad ev(ec')=(z, c?x)
\quad c \in UC^{in}
$}
{}
}
\LeftLabel{
    % (R7) $\emph{INC}^{specUncI}$
    (R7) $\emph{INC}^\uncIn_\spec$
%\stackanchor{{\bf R6 Specified uncontrollable}}{{\bf input outside $tp$}}
}
\UnaryInfC{
\stackanchor{$\big(
      ec
\;,\; c?x
\;,\; \phi^\obs_\spec
\;,\; \emptyset
\;,\; id_{\widehat{A}} 
\;,\; \emph{INC}^\uncIn_\spec\big) \in \widehat{Tr}
$}
{
%$\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
}
}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.75}
\AxiomC{
\stackanchor{$
      ec \in \mathbb{EC}(tp)
\quad ev(ec)=(z, c?x)
\quad c \in UC^{in}
$}
{}
}
\LeftLabel{
    % (R8) $\emph{INC}^{unspecUncI}$
    (R8) $\emph{INC}^\uncIn_\unspec$
%\stackanchor{{\bf R7 Under-specified}}{{\bf uncontrollable input}}
}
\UnaryInfC{
\stackanchor{$\big(
      ec
\;,\; c?f^{in}_c(ec)
\;,\; \phi^\obs_\unspec
\;,\; \emptyset
\;,\; id_{\widehat{A}} 
\;,\; \emph{INC}^\uncIn_\unspec\big) \in \widehat{Tr}
$}
{
%$\phi^\obs_\unspec =  (f^{dur} (ec) < \emph{TM} ) \land  \bigwedge_{\substack{pec(ec') =ec \\ chan(ec')=c }}(\forall F^{ini}.\neg\pi(ec'))$
}
}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.75}
\AxiomC{
\stackanchor{
    $ec \in \mathbb{EC}(tp)$
}
{}
}
\LeftLabel{
    (R9) $\emph{INC}^{dur}$
%\stackanchor{{\bf R8 Specified quiescence}}{{\bf }}
}
\UnaryInfC{
\stackanchor{$\big(
      ec
\;,\; \delta!
\;,\; \phi^{\delta}_\spec
\;,\; \emptyset
\;,\; id_{\widehat{A}}
\;,\; \emph{INC}^{dur}\big) \in \widehat{Tr}
$}
{
$
    \phi^{\delta}_\spec = f^{dur}(ec) \geq \emph{TM}
    \land \bigvee_{\substack{pec(ec')=ec 
        \\ chan(ec') \in C^{out} \cup UC^{in} \cup \{\delta\}}} \exists F^{ini}.\pi(ec')
$
}}
\end{scprooftree}
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.75}
\AxiomC{\stackanchor{$ec \in \mathbb{EC}(tp)$}{}}
\LeftLabel{ (R10) $\emph{FAIL}^{dur}$
%\stackanchor{{\bf R9 Unspecified quiescence}}{{\bf }}
}
\UnaryInfC{
\stackanchor{$\big(
      ec , \delta!%\emph{TM}
\;,\; \phi^\delta_\unspec
\;,\; \emptyset
\;,\; id_{\widehat{A}} 
\;,\; \emph{FAIL}^{dur}\big)
    \in \widehat{Tr}
$}
{
$\phi^{\delta}_\unspec = f^{dur}(ec) \geq \emph{TM}
    \land \bigwedge_{\substack{pec(ec')=ec 
        \\ chan(ec') \in C^{out} \cup UC^{in} \cup \{\delta\}}} \forall F^{ini}.\neg \pi(ec')$
}}
\end{scprooftree}
\end{minipage}

% \begin{minipage}{11cm}
% \centering
% \begin{scprooftree}{.75}
% \AxiomC{\stackanchor{$ec \in \mathbb{EC}(tp)$}{}}
% \LeftLabel{ (R10) $\emph{FAIL}^{dur}$
% %\stackanchor{{\bf R9 Unspecified quiescence}}{{\bf }}
% }
% \UnaryInfC{
% \stackanchor{
% $\big(
%       ec
% \;,\; \delta!%\emph{TM}
% \;,\; \phi^\delta_\unspec
% \;,\; \emptyset
% \;,\; id_{A_{\emph{TC}}}
% \;,\; \emph{FAIL}^{dur}
% \big) \in Tr_{\tc}$}{
% \stackanchor{
%  $\phi^\delta_\unspec= f^{dur}(ec) \geq \emph{TM} \land
% \psi^\obs_\unspec$}
% {\stackanchor
% {$ \psi^\obs_\unspec=
%     \bigwedge{\substack{pec(ec')=ec \\ chan(ec') \in C^{out}}} \forall F^{ini}.\forall f^{out}_{chan(ec')}.\neg\pi(ec')
% $}
% {$ \land \bigwedge_{\substack{pec(ec')=ec \\ chan(ec') \in UC^{in}}} \forall F^{ini}. \forall f^{in}_{chan(ec')} . \neg \pi(ec')
% $}
% }
% }}
% \end{scprooftree}
% \end{minipage}
}
%\commental{La symétrie requise par mon biais cognitif ! :-)} \commentbb{Done + correction!}

% $\begin{array}{rllll}
%     \psi^\obs_\unspec =
%     &
%     \bigwedge{\substack{pec(ec')=ec \\ chan(ec') \in C^{out}}}
%     &
%     \forall F^{ini} .
%     &
%     \forall f^{out}_{chan(ec')} .
%     &
%     \neg\pi(ec')
% \\
%     \land
%     &
%     \bigwedge_{\substack{pec(ec')=ec \\ chan(ec') \in UC^{in}}}
%     &
%     \forall F^{ini}.
%     &
%     \forall f^{in}_{chan(ec')} .
%     &
%     \neg \pi(ec')
% \end{array}$

\end{definition}

%Generally speaking, 
A verdict $\text{PASS}$ is reached when $tp$ is covered, verdicts of the form $\text{INC}^m_n$ are reached when traces deviate from $tp$ while remaining in $\mathbb{G}$ and verdicts of the form $\text{FAIL}^m$ stand for traces outside $\mathbb{G}$. The annotations $n$ and $m$ provide additional information on the cause of the verdict. 
Rules $R1$, $R2$ and $R6$, grouped together under the label $\text{SKIP}$, allow advancing along $tp$, resp. by stimulating $LUT$ with the sending of data, observing an emission on $C^{out}$ and observing a reception on $UC^{in}$. Rule $R3$ (with the label $\text{PASS}$) indicates that the last EC of $tp$, thus the $\text{PASS}$ verdict, has been reached. Rules $R4$, $R7$, $R8$ and $R9$, each with a label of the form $\text{INC}^m_n$ indicate that the last observed event causes $LUT$ to leave $tp$, without however leaving $\mathbb{G}$, resp. by observing an output, an input specified in $\mathbb{G}$, an input not specified in $\mathbb{G}$ and a time-out observation. Lastly, rules $R5$ and $R10$, resp. labelled by  $\text{FAIL}^{out}$ and $\text{FAIL}^{dur}$, raise a $\text{FAIL}$ verdict, for resp. an unauthorized output and an exceeded time-out.

%We will comment more in details on the different rules and verdicts using Ex.~\ref{ex:test-case}. %Execution contexts of $tp$ become states of the test case except $tgt(tp)$ which is replaced by $\text{PASS}$. Every verdict state is connected to one or more contexts of $tp$:  Specified output, e.g., transition from $ec_2$ to $\text{INC}^{out}$ inferred from $ec_{10}$, specified uncontrollable input, e.g., transition from $ec_1$ to $\text{INC}^\uncIn_\spec$ inferred from $ec_9$, underspecified uncontrollable input ($\text{INC}^\uncIn_\unspec$), unspecified output ($\text{FAIL}^{out}$), and unspecified quiescence ($\text{FAIL}^{dur}$).



\begin{example}
\label{ex:test-case} In Fig.~\ref{fig:test_case_ATM}, the test case for $tp=ec_0ec_1\ldots ec_5$ (see Ex.~\ref{ex:tiosts-determ}) is depicted. Certain verdict states are repeated for readability, and defining rules annotate the transitions. The test case utilizes the $\text{Wdral}$ channel as a controllable input channel for stimulation while observing all other channels. For space considerations, we comment only on some rules.

 \noindent Rule $R1$ defines a stimulation action $\actOut{Wdral}\f{amt_1}$ (transition from $ec_1$ to $ec_2$) constrained by $\pi(tp)$ to select an appropriate value for $\f{amt_1}$ together with a time of stimulation $\f{z_1}$ that allows to remain within the test purpose. Within $\pi(tp)$, $\f{amt_1}$ is limited to the range $10\leq \f{amt_1} \leq 500$, while $\f{z_1}$ remains unconstrained (a duration measured with clock $\f{z_1}$, following the previous observation $\actIn{Init}$). It is worth noting that all non-revealed variables, i.e., other than $\f{z_0}$, $\f{z_1}$, and $\f{amt_1}$, appearing in $\pi(tp)$ are bound by the existential quantifier due to their unknown values at this stage of execution. Finally, the clock $\f{z_2}$ is reset to enable reasoning on subsequent actions' duration (measured on $\f{z_2}$).

\noindent  Rule $R2$ defines an observation action $\actIn{Debit}(\f{\freshOut{1}{D}{1}},\f{\freshOut{1}{D}{2}},\f{\freshOut{1}{D}{3}})$  constrained by 
$(\f{z_2}\!<\!\maxWaitingBound) 
\wedge \exists \f{fee_0} . \piAlias{3}$ (transition from $ec_2$ to $ec_3$) while rule $R5$ defines the same observation constrained by 
 $(\f{z_2}\!<\!\maxWaitingBound)
    \land \forall \f{fee_0} .
    \neg \, \piAlias{3}
    \land \forall \{ \f{fee_0} \} \, . \,
    \neg \, \piAlias{10}
    $ (transition from $ec_2$ to $\text{FAIL}^{out}$). Both situations are possible which shows from the following traces (the latter two diverge %from the test purpose
due to data resp. time non-compliance): 
    
    $(0,\actIn{Init}) .
    (0,\actOut{Wdral}50) .
    (0,\actIn{Debit}(1,51,\ATMID))$ reaches $ec_3$
    
    $(0,\actIn{Init}) . 
    (0,\actOut{Wdral}50) .
    (0,\actIn{Debit}(1,0,\ATMID)$ reaches $\text{FAIL}_{out}$ 
    
    $(0,\actIn{Init}) . 
    (0,\actOut{Wdral}50) .
    (2,\actIn{Debit}(1,51,\ATMID))$ reaches $\text{FAIL}_{out}$


\noindent Rule $R6$ defines an unspecified quiescence $\delta!$ constrained by $(\f{z_2} \geq \maxWaitingBound)
    \land %\big(
    \forall \f{fee_0} \, . \neg \piAlias{3}
    \land
    \forall \f{fee_0} \, . \neg \piAlias{10}
    \land
    \forall \f{fee_0} \, .\neg \piAlias{11}
    % \big)
$ (transition from $ec_2$ to $\text{FAIL}^{dur}$). This situation arises in the trace $(0,\actIn{Init}).(0,\actOut{Wdral}50).(5,\delta!)$, where time-out $\maxWaitingBound$ is set to $5$. In this case, the time-out is triggered without the mandatory output on the channel $\text{Debit}$ being observed. 

\noindent Rule $R9$ defines a specified quiescence $\delta!$ (transition from $ec_2$ to $\text{INC}^{dur}$ not drawn for space). This situation arises when there is still sufficient time to reach $ec_3$, $ec_{10}$ or $ec_{11}$ (n.b., no quiescence enrichment applies from $ec_2$, see Ex.~\ref{ex:quiescence}).
%for some trace $(0,\actIn{Init}).(0,\actOut{Wdral}50).(0,\delta!)$.
%\commentbb{SAY TEST CASE IS COMPLETE ON WHAT IT OBSERVES (OUT and UncINPUT)}
\end{example}
% that we cannot detail due to lack of space.

%\subsection{Soundness of test cases}
%In the meantime, will discuss how a test case can support test execution. %First, 
%Let us point out that by construction,  $\widehat{Q} \subseteq \mathbb{EC}(tp) \cup \mathbb{V}$ since the elements of $\mathbb{EC}(tp) \setminus \{ tgt(tp) \}$ are in %$\widehat{V}$
%$\widehat{Q}$ and the only other elements added are in $\mathbb{V}$, and thus are %leaves
%sink states of the test case $\mathbb{TC}$. So, the only states with a successor in $\mathbb{TC}$ are in $\mathbb{EC}(tp) \setminus \{ tgt(tp) \}$. 

\begin{figure}[t] %[h!]
    \centering
    %\makebox[.9\textwidth][c]{
    
    \resizebox{1\textwidth}{!}{
        \hspace{-1cm}\input{fig/tikz_atm_testcase_simplif}
    }
	\caption{Test case for $\text{ATM}$}
% Tentative version simplifiée pour la lisibilité.
	\label{fig:test_case_ATM}
 \vspace{-.5cm}
\end{figure}

A test case  $\mathbb{TC}$ interacts with a $LUT$, designed to comply with a TIOSTS $\mathbb{G}$, to issue a verdict concerning a test purpose $tp$. $\mathbb{TC}$ is therefore defined as a mirror image of $\mathbb{G}$: emissions (receptions) in $\mathbb{TC}$ correspond to receptions (emissions) of $\mathbb{G}$ (cf. rules $R1$ and $R2$), except uncontrollable channels whose actions are not reversed (cf rule $R6$). Given a concrete action $act$ (with $v$ for value received or sent), we denote $\overline{act}$ its mirror action, defined as follows: $\overline{c!v} = c?v$ for $c \in C^{out}$, $\overline{c?v} = c!v$ for $c \in CC^{in}$ and  $\overline{c?v} = c?v$ for $c \in UC^{in}$.
We introduce an execution relation that abstracts a synchronized execution of a trace with $\mathbb{TC}$: 
\begin{definition}[Relation execution $\leadsto_{\mathbb{TC}}$]
Let $\mathbb{G}$ be a TIOSTS and $tp$ a test purpose for $\mathbb{G}$ with $\mathbb{TC} = (\widehat{Q},\widehat{q_0},\widehat{Tr})$ the test case guided by $tp$.

The \emph{execution relation}  $\leadsto_{\mathbb{TC}}\subseteq \big( Evt(C_\delta)^* \times  \widehat{Q} \times M^F \big)^2$  is defined by:

for $ev.\sigma \in Evt(C_\delta)^*$, $q,q' \in \widehat{Q}$ and for $\nu, \nu' \in M^F$, $(ev.\sigma,q,\nu) ~\leadsto_{\mathbb{TC}}~ (\sigma, q',\nu')$ holds iff there exists $tr\in \widehat{Tr}$ s.t. $src(tr)\!=\! q$, $tgt(tr)\!=\!q'$, $\nu'(act(tr))=\overline{act(ev)}$ and $M \models_{\nu'} \phi(tr)$ with $\nu'$ defined as:
 \begin{itemize}
     \item if $ev\!=\!(d,c?v)$ and $chan(tr)\!=\!c$ then $\nu'\!=\!\nu[f^{dur}(q)\!\mapsto\!d][ f^{in}_c(q)\!\mapsto\!v]$ ;
     \item if $ev\!=\!(d,c!v)$ and $chan(tr)\!=\!c$ then $\nu'\!=\!\nu[f^{dur}(q)\!\mapsto\!d][f^{out}_c(q) \!\mapsto\! v]$ :
     \item else, i.e., $ev\!=\!(d,\delta!)$ and $chan(tr)\!=\!\delta$, $\nu'=\nu[f^{dur}(q)\!\mapsto\!d]$.
 \end{itemize}
 \end{definition}


%Let $LUT$ a subset of $ Evt(C_\delta)^*$ satisfying ${\cal H}$. 
%We introduce an execution relation that abstracts a synchronized execution of a $LUT$, given as a subset of $Evt(C_\delta)^*$ satisfying ${\cal H}$, and the test case $\mathbb{TC}$: 
%\vspace{-.275cm}
%\[\leadsto_{\mathbb{TC}}\subseteq \big( Evt(C_\delta)^* \times  \widehat{Q} \times M^F \big)^2  \] 
%\vspace{-.575cm}

Intuitively, a step $(ev.\sigma, q,\nu) ~\leadsto_{\mathbb{TC}}~ (\sigma, q',\nu')$ consists in:
\begin{itemize}
    \item reading the first element $ev$ of a trace from a test case state $q$ and an interpretation $\nu$  synthesizing the known information about the variables in~$F$
    \item finding a transition $tr$ in $\widehat{Tr}$ whose action matches the mirror action of $ev$ 
    \item building a new triple with $\sigma$ the trace remaining to be read, $q'$ a successor state of $q$ in $\widehat{Q}$, and $\nu'$ the updated interpretation of the variables~$F$. 
\end{itemize}
The execution relation simulates a parallel composition between timed input output systems, synchronizing inputs and outputs. Our formulation deviates from the one in \cite{KrichenT06} for two essential reasons: the symbolic nature of the test case requires the intermediate interpretations of variables to be memorized, and uncontrollable channels require the synchronization to be adapted \cite{EscobedoGGC10}.
Let $LUT$ be a subset of $ Evt(C_\delta)^*$ satisfying ${\cal H}$ and $\overset{*}{\leadsto}_{\mathbb{TC}}$ be the reflexive and transitive closure of  $\leadsto_{\mathbb{TC}}$. Given a $LUT$ trace $\sigma_0$, we apply the execution relation iteratively from an initial triplet consisting of $\sigma_0$, $ec_0$ an initial EC and $\nu_0$ an arbitrary interpretation, to obtain the corresponding test verdict for $tp$, so that the verdict set obtained from the execution of $\mathbb{TC}$ on $LUT$ is defined by: 

%\noindent $vdt(LUT,\mathbb{TC})= \bigcup_{\substack{\sigma_0\in LUT ,\; \nu_0 \in M^F \\ \text{V}\in\mathbb{V}}}\{\text{V} ~|~ (\sigma_0,{q_0}_{\tc}, \nu_0) \overset{*}{\leadsto}_{\mathbb{TC}} (\sigma,\text{V}, \nu )\}$. 

\noindent $vdt(LUT,\mathbb{TC})= \{\text{V} ~|~ \exists \sigma_0 \in LUT, \nu_0 \in M^F, \text{V} \in \mathbb{V}, (\sigma_0,{q_0}_{\tc}, \nu_0) ~\overset{*}{\leadsto}_{\mathbb{TC}} (\sigma,\text{V}, \nu )\}$. 


\noindent Th.~\ref{th:corr} states the soundness of test case execution for the verdicts $\text{FAIL}^m$ (see proof in Appendix~\ref{anx:proof}).

\begin{theorem}
\label{th:corr} 
Let $C$ be a set of channels. Let $\mathbb{G}$ and $LUT$ be resp. a TIOSTS defined on $C$ and a subset of $Evt(C_\delta)^*$ satisfying $\cal{H}$. \\
 If $LUT~tioco~\mathbb{G}$ then for any test purpose $tp$ for $\mathbb{G}$ with $\mathbb{TC}$ as test case guided by $tp$, we have $\emph{FAIL}^{out}\not\in vdt(LUT, \mathbb{TC}) $ and $\emph{FAIL}^{dur}\not\in vdt(LUT, \mathbb{TC})$.
\end{theorem}



Our test cases can be executed by designing a test program that maintains the following elements: (1) a current state of the test case, some execution context $ec$ (unique by trace-determinism), which is updated by following a test case transition $tr$ corresponding to applied stimulations or processed observations, and (2) a current interpretation $\nu$ that is significant for the revealed variables so-far (from the set $\overline{f}(ec)$). The interpretation $\nu$ is used to evaluate transition guards (whether $M \models_\nu \phi(tr)$) to determine the stimulation's value and the time to send the value or to check observation's value and occurrence time. The test program terminates when a verdict state of the test case is reached. 

{\em Implementation issues.} The test case generation is implemented as module in the Diversity symbolic execution platform~\cite{diversity}. Resulting test cases are expressed in Diversity's entry language, allowing their exploration through symbolic execution with the SMT-solver Z3~\cite{Z3}. 
%to verify the reachability of divergent transitions. 
%We minimize the test cases by keeping only reachable transitions. 
For easier execution, we export the test cases from Diversity in JSON format, with transition guards expressed in the SMT-LIB input format for SMT-solvers. We applied the test case generation module to the ATM example on an Intel Core i7. Throughout the experiment, we varied the size of the test purposes, measured in transitions of the reference TIOSTS, ranging from $5$ (discussed in Ex.~\ref{ex:test-case}) to $10$, \ldots, $100$. Our module successfully verified trace-determinism for all test purposes. However, we noticed a significant increase in generation duration as the test purpose size increased, while still remaining practicable. Specifically, generating the TIOSTS test case ($513$ transitions) for the test purpose of $100$ transitions took more than $40$s, in contrast to only $500$ms for the test purpose of size $5$ ($31$ transitions) resp. $8$s for the test purpose of size $50$ ($138$ transitions).


%A simple way of executing our test cases is to design a test program which maintains {\bf{\em (1)}} a current state issued from the test case, i.e., some execution context $ec$ (unique by trace-determinism), which is updated by following some test case transition $tr$ corresponding to a stimulation it applies or an available observation it processes, and {\bf{\em (2)}} a current interpretation $\nu$ significant for the revealed variables so-far, those from the set $\overline{f}(ec)$ that is used to assess transitions' guards (whether $\nu \models \phi(tr)$). The transitions' guards are used to compute stimulations and their submission time (obtained by solving $\phi(tr)$ and remembered through $\nu$) %(proposed by the solver) or to verify observations and their occurrence time (matched through $\nu$ that is checked to satisfy $\phi(tr)$). The test program terminates whenever a verdict state of the test case is reached. We have implemented our test case generation as a module of the symbolic execution platform Diversity~\cite{diversity}.
%A generated test case is expressed in Diversity's entry language as for the reference TIOSTS which allows its exploration by symbolic execution coupled with SMT-solver Z3~\cite{Z3}, e.g., to check the reachability of divergent transitions. We reduce (minimize) the test case to only those reachable transitions. To ease test cases execution, we have exported them from Diversity in the JSON format where test case transitions' guards are expressed in the input format for SMT-solvers, called SMT-LIB.

%We have implemented our test case generation as a module of the symbolic execution platform Diversity~\cite{diversity}. A generated test case is expressed in Diversity xLIA modeling language as for the reference TIOSTS. The test case can then be animated by symbolic execution in Diversity, e.g., to verify the reachability of divergent transitions. Constraint solving required in symbolic execution is done thanks to the SMT-solver Z3~\cite{}. If some divergent transitions are not reachable, we remove them from the test case and reduce (minimize) it to only those reachable transitions. To ease test execution, we have exported it from Diversity in the JSON format where the test case transitions' guards are expressed in the input format for SMT-solvers, called SMT-LIB.










==> 5_testcase-old2.tex <==

%\subsection{Path-guided test case}
%\noindent {\bf Test case generation} 
Roughly speaking, a test case $\mathbb{TC}$ will be a mirror TIOSTS of a TIOSTS $\mathbb{G}$, restricted by $tp$, a test purpose of $\mathbb{G}$, intended to interact with a $LUT$ that we wish to check its conformance to $\mathbb{G}$ up to $tp$.
$\mathbb{TC}$ will be a tree-like TIOSTS with $tp$ of $\mathbb{G}$ as a backbone, incorporating the following specific characteristics:
%We will define a test case as a TIOSTS-like structure with a test purpose $tp$ as the backbone. More exactly, a test case will be a tree-like structure with the following particularities:
\begin{itemize}
    \item execution contexts in $\mathbb{EC}(tp)$ constitute the main branch,
    \item sink states or leaves are assimilated with a test verdict. Notably, the last execution context $tgt(tp)$ of $tp$ will be assimilated with the $\text{PASS}$ verdict,
    \item from each $ec$ in $\mathbb{EC}(tp)$ other than $tgt(tp)$, the outgoing arcs outside $tp$ decline all ways to deviate from $tp$ and directly lead to a verdict state, either an inconclusive verdict or a failure verdict.
    %\\ \commental{$\mathbb{EC}(tp)$ est requis (?) dans les règles !} \commentplg{J'ai mis dans les règles $(\mathbb{EC}(\mathbb{G}) \setminus  \mathbb{EC}(tp))$}
\end{itemize}    


In Def.\ref{def:test-case}, we define $\mathbb{TC}$ by enumerating the different cases of transitions to be built according to channel type and $tp$ membership. We now give a few indications for enhancing the definition readability. Channel roles are reversed: channels in $CC^{in}$ as well as %the particular
channel $\delta$ (resp. $C^{out} \cup UC^{in}$) become output (resp. input) channels. 
%Transitions from $tp$ on $CC^{in}$ are emission transitions in $\mathbb{TC}$, and symmetrically, transitions from $tp$ on $C^{out} \cup UC^{in}$ are receptions in $\mathbb{TC}$. 
Variables of $\mathbb{TC}$ will be 
 symbolic variables involved in $tp$ and will be used to store successive concrete events observed on $LUT$. Any observation  on $LUT$ will be encoded as an input transition in $\mathbb{TC}$, whether it is an emission from a channel of $C^{out}$, a reception on a channel of $UC^{in}$ or a time-out observation. On the latter, it is conventional to consider that a system that does not react before a certain delay, chosen to be long enough, is in a state of quiescence. The only notable exception is when input transitions of $tp$ give rise to output transitions for $\mathbb{TC}$, modeling a situation in which $\mathbb{TC}$ stimulates $LUT$ by sending it data. The choice of the data to send is conditioned by two constraints: (i) taking into account the information collected so far and stored in the variables of $\mathbb{TC}$ in the first steps, and (ii) the guarantee of being able to reach the last EC of $tp$, i.e. the verdict $\text{PASS}$. This will be done by ensuring the satisfiability of the path condition of $tp$, leaving aside the variables already binded. 
%The process of test case generation will be applied to the fully-prepared symbolic subtree containing ECs of the test purpose $tp$ denoted by $\mathbb{EC}(tp)$ and adjacent ECs $\mathbb{EC}_a(tp)$. The trace-deterministic property of $tp$ is verified for the execution contexts from this fully-prepared subtree as stated in Def~\ref{def:Test purpose} which is a perquisite to the following  test case definition.
% The process of test case generation will be applied to a fully-prepared symbolic subtree containing ECs of the test purpose $tp$ denoted by $\mathbb{EC}(tp)$ and adjacent ECs $\mathbb{EC}_a(tp)$. These are successors of the ECs composing $tp$ from which we exclude those of $tgt(tp)$, and any successor $ec$ with a controllable input,.i.e., $chan(ec)\in CC^{in}$ . Obviously, we also require $Sat(\pi(ec))$ for any $ec \in \mathbb{EC}_a(tp)$. As we restrict to trace-deterministic TIOSTS, we check Def.~\ref{def:Deterministic_TIOSTS} for execution contexts from this fully-prepared subtree.
%Finally, we consider a global maximal waiting-time denoted as a constant $\emph{TM}$, in order to bound the waiting delay for observing outputs or internal inputs emitted by other systems. The waiting-time fixed in the test case to avoid waiting for too long for such observations. For instance, it can be chosen as the maximal value among those which bound the occurrences of observations (outputs or uncontrollable inputs) in the definition of the test purpose.%, plus some duration.

We will refer to variables of a symbolic path as follows: for\footnote{For $i$ and $j$ in $\mathbb{N}$ verifying $i < j$, $[i,j)$ contains the integers from $i$ to $j-1$ included.} $\alpha \in \{in,out\}$, $f^\alpha(p)=\bigcup_{i \in [1,n)} f^\alpha(ec_i)$ will denote all introduced fresh variables in $F^\alpha$ used to compute a symbolic path $p =ec_0.ec_1\ldots ec_n$. Similarly, $f^{dur}(p) = \{ f^{dur}(ec_i) | i \in [1,n) \}$. Moreover, for a target execution context $ec_n = tgt(p)$, we denote $\overline{f}^\alpha(ec_n)$ and $\overline{f}(ec_n)$ resp. for $f^\alpha(p)$ and  $f(p)$. 

\begin{definition}[Path-guided test case]
\label{def:test-case}
Let $tp$ be a test purpose for a TIOSTS $\mathbb{G}$. 
Let us consider the signature $\widehat{\Sigma} = (\widehat{A}, \widehat{K}, \widehat{C})$ where: 
\begin{itemize}
    \item $\widehat{A} = f^{in}(tp) \cup f^{out}(tp)$, 
    \item $\widehat{K}=f^{dur}(tp)$, 
    \item $\widehat{C}=C_\delta$ such that $\widehat{C}^{in} = C^{out} \cup UC^{in}$ and $\widehat{C}^{out} = CC^{in} \cup \{\delta\}$
\end{itemize}    
A \emph{test case guided by} $tp$ is a TIOSTS $\mathbb{TC}=(\widehat{Q}, \widehat{q_0}, \widehat{Tr})$ over $\widehat{\Sigma}$ where: %where: $A_{\tc} = f^{in}(tp) \cup f^{out}(tp)$, $K_{\tc}=f^{dur}(tp)$, $C_{\tc}=C \cup \{\delta\}$ such that ${(C_{\tc})}^{in} = C^{out} \cup UC^{in}$ and ${(C_{\tc})}^{out} = CC^{in} \cup \{\delta\}$,  
\begin{itemize}
    \item $\widehat{Q} = \big(\mathbb{EC}(tp) \setminus \{tgt(tp)\} \big) \cup \mathbb{V}$ where: \\
    %~\footnote{Verdicts $\text{FAIL}^{out}$ and $\text{FAIL}^{dur}$ mean non-conformance w.r.t. tioco} 
    $\mathbb{V} = \{$
    $\emph{PASS},$
    $\emph{FAIL}^{out},$
    $\emph{FAIL}^{dur},$
    $\emph{INC}^{out},$
    $\emph{INC}^{dur},$
    % $\emph{INC}^{specUncI},$
    $\emph{INC}^\uncIn_\spec,$
    % $\emph{INC}^{unspecUncI}\},$
    $\emph{INC}^\uncIn_\unspec$
$\}$,
    \item $\widehat{q_0}=ec_0$,
    \item $\widehat{Tr}$ is defined by a set ${\cal R}$ of  10 rules of the form $(Ri)$ LABEL $\frac{H}{ tr\in  \widehat{Tr}}$ for $i \in [1,10]$. Such a rule reads as follows: the transition $tr$ can be added due to rule $Ri$ to $\widehat{Tr}$ provided that hypothesis $H$ holds and $Sat(tr)$.
\end{itemize}   

In writing the rules of ${\cal R}$, we will use the following formulas 

\resizebox{!}{55pt}{
$\begin{array}{lcl}
&\\
    \phi_{stim} &:&
    \exists F^{ini} \cup \overline{f}(tgt(tp)) %Var(\pi(tp))
    \setminus \overline{f}(ec'). \pi(tp) 
\\
&
\\
\phi^\obs_\spec &:&
    %(z < \emph{TM})
    f^{dur} (ec) < \emph{TM}
    \wedge (\exists F^{ini}.\pi(ec'))
\\
\phi^\obs_\unspec &:&
        f^{dur} (ec) < \emph{TM}  \land  \bigwedge_{\substack{pec(ec') = ec \\ chan(ec')=c }}(\forall F^{ini}.\neg\pi(ec'))
\\
&
\\
\phi^{\delta}_\spec &:& 
f^{dur}(ec) \geq \emph{TM}
    \land \bigvee_{\substack{pec(ec')=ec 
        \\ chan(ec') \in C^{out} \cup UC^{in} \cup \{\delta\}}} (\exists F^{ini}.\pi(ec'))
\\
%\centerline{
\phi^{\delta}_\unspec &:& 
f^{dur}(ec) \geq \emph{TM}
    \land \bigwedge_{\substack{pec(ec')=ec 
        \\ chan(ec') \in C^{out} \cup UC^{in} \cup \{\delta\}}} (\forall F^{ini}.\neg \pi(ec'))
\\
&
\end{array}
$ }

% that occur several times in the rules
% and 
where the constant $\emph{TM}$ (Time-out) %limits the 
sets the maximum waiting-time for observing outputs or uncontrollable inputs. %The waiting-time fixed in the test case to avoid waiting for too long for such observations.
    


\vspace{.2cm}


{
\centering
\begin{minipage}{10cm}
\centering
\begin{scprooftree}{.76}
\AxiomC{$
      ec\xrightarrow[]{(z, c?x)} ec' \in \mathbb{EC}(tp)
%\;\; pec(ec')=ec \;\; ev(ec') = (z, c?x)
\;\; c \in CC^{in}
$}
\LeftLabel{
   $\begin{array}{r}(R1) \\ \emph{SKIP} \end{array}$
}
\UnaryInfC{
\stackanchor{ $\big(
      ec
, c!x
, \phi_{stim}
, \{ f^{dur} (ec) \}
, id_{\widehat{A}}
, ec'
\big) \in \widehat{Tr}$ }{
% $\phi_{stim} =
%     (\exists F^{ini} \cup \overline{f}(tgt(tp)) %Var(\pi(tp))
%     \setminus \overline{f}(ec'). \pi(tp) )
% $
}
}
\end{scprooftree}
\end{minipage}

\hspace{.3cm}\begin{minipage}{0.5\linewidth}%{9cm}
\centering
\begin{scprooftree}{.76}
\AxiomC{
\stackanchor{$
       ec\xrightarrow[]{(z, c!y)} ec' \in \mathbb{EC}(tp)
$}
{
$
ec' \neq tgt(tp)
\;\; c \in C^{out}
$
}
}
\LeftLabel{
     $\begin{array}{r}(R2) \\ \emph{SKIP} \end{array}$
%\stackanchor{{\bf R2 Specified output}}{{\bf inside $tp$}}
}
\UnaryInfC{
$\big( ec
, c?y
, \phi^\obs_\spec
, \{ f^{dur} (ec') \}
, id_{\widehat{A}}
, ec' \big) \in \widehat{Tr}$ 
}
\end{scprooftree}
\end{minipage}
\begin{minipage}{0.45\linewidth}
\centering
\begin{scprooftree}{.76}
\AxiomC{
\stackanchor{$
      ec\xrightarrow[]{(z, c!y)} ec' \in \mathbb{EC}(tp)
$}
{$ec' = tgt(tp)
\;\; c\in C^{out}
$}
}
\LeftLabel{
$\begin{array}{r}(R3) \\ \emph{PASS} \end{array}$
% \stackanchor{
% {\bf R2 Specified output}}{{\bf inside $tp$ (last)}}
}
\UnaryInfC{
\stackanchor{$\big(
     ec
, c?y
, \phi^\obs_\spec
, \emptyset
, id_{\widehat{A}}
, \emph{PASS} \big) \in \widehat{Tr}
$}
{
% $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
}
}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\hspace{-.3cm}\begin{minipage}{0.465\linewidth}
\centering
\begin{scprooftree}{.76}
\AxiomC{\stackanchor{$
%    ec \in (\mathbb{EC}(\mathbb{G}) \setminus  \mathbb{EC}(tp))
 ec\xrightarrow[]{(z, c!y)} ec'
\;\; ec \in \mathbb{EC}(tp) \setminus \{tgt(tp)\}
$}
{
$ec' \in \mathbb{EC}(\mathbb{G})
\;\; c \in C^{out}
$
}
}
\LeftLabel{
$\begin{array}{r}(R4) \\ \emph{INC}^{out} \end{array}$
%\stackanchor{{\bf R3 Specified output}}{{\bf outside $tp$}}
}
\UnaryInfC{$\big(
      ec
, c?y
, \phi^\obs_\spec
, \emptyset
, id_{\widehat{A}}
, \emph{INC}^{out}\big) \in \widehat{Tr}
$}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}
\begin{minipage}{.5\linewidth}
\centering
\begin{scprooftree}{.76}
\AxiomC{\stackanchor{$
\textcolor{white}{ec\xrightarrow[]{(z, c!y)} ec'
\;\; ec \in \mathbb{EC}(tp) \setminus \{tgt(tp)\}}   
$}
{
$
ec \in \mathbb{EC}(tp)
\;\; c \in C^{out}
$
}
}
\LeftLabel{
$\begin{array}{r}(R5) \\ \emph{FAIL}^{out} \end{array}$
%\stackanchor{{\bf R4 Unspecified output}}{{\bf}}
}
\UnaryInfC{
$\big(
      ec
, c?f^{out}_c(ec)
, \phi^\obs_\unspec
, \emptyset
, id_{\widehat{A}}
, \emph{FAIL}^{out}\big) \in \widehat{Tr}$}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\hspace{-.2cm}\begin{minipage}{0.49\linewidth}%{9cm}
\centering
\begin{scprooftree}{.76}
\AxiomC{\stackanchor{$
ec\xrightarrow[]{(z, c?x)} ec' \in  \mathbb{EC}(tp)
$}
{
$
c \in UC^{in}  
$
}
}
\LeftLabel{
$\begin{array}{r}(R6) \\ \emph{SKIP} \end{array}$
}
\UnaryInfC{
\stackanchor{$\big(
      ec
, c?x
, \phi^\obs_\spec
, \{ f^{dur} (ec') \}
, id_{\widehat{A}}
, ec' \big) \in \widehat{Tr}$}
{
%$\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
}
}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}
\begin{minipage}{0.47\linewidth}
\centering
\begin{scprooftree}{.76}
\AxiomC{
\stackanchor{$
ec\xrightarrow[]{(z, c?x)} ec'
\;\; ec \in  \mathbb{EC}(tp) \setminus \{tgt(tp)\}
$}
{$\;\; ec' \in \mathbb{EC}(\mathbb{G})
\;\; c \in UC^{in}
$}
}
\LeftLabel{
   $\begin{array}{r}(R7) \\ \emph{INC}^\uncIn_\spec \end{array}$
%\stackanchor{{\bf R6 Specified uncontrollable}}{{\bf input outside $tp$}}
}
\UnaryInfC{
\stackanchor{$\big(
      ec
, c?x
, \phi^\obs_\spec
, \emptyset
, id_{\widehat{A}} 
, \emph{INC}^\uncIn_\spec\big) \in \widehat{Tr}
$}
{
%$\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
}
}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\begin{minipage}{11cm}
\centering
\begin{scprooftree}{.76}
\AxiomC{
\stackanchor{$
      ec \in \mathbb{EC}(tp)
%\;\; ev(ec)=(z, c?x)
\;\; c \in UC^{in}
$}
{}
}
\LeftLabel{
   $\begin{array}{r}(R8) \\ \emph{INC}^\uncIn_\unspec \end{array}$
%\stackanchor{{\bf R7 Under-specified}}{{\bf uncontrollable input}}
}
\UnaryInfC{
\stackanchor{$\big(
      ec
, c?f^{in}_c(ec)
, \phi^\obs_\unspec
, \emptyset
, id_{\widehat{A}} 
, \emph{INC}^\uncIn_\unspec\big) \in \widehat{Tr}
$}
{
%$\phi^\obs_\unspec =  (f^{dur} (ec) < \emph{TM} ) \land  \bigwedge_{\substack{pec(ec') =ec \\ chan(ec')=c }}(\forall F^{ini}.\neg\pi(ec'))$
}
}
\end{scprooftree}
%with $\phi^\obs_\spec = (f^{dur} (ec) < \emph{TM}) \wedge (\exists F^{ini}.\pi(ec))$
\end{minipage}

\vspace{.2cm}

\hspace{-.735cm}\begin{minipage}{0.5\linewidth}%{9cm}
\centering
\begin{scprooftree}{.76}
\AxiomC{
\stackanchor{
    $ec \in \mathbb{EC}(tp)$
}
{}
}
\LeftLabel{
$\begin{array}{r}(R9) \\ \emph{INC}^{dur}\end{array}$
%\stackanchor{{\bf R8 Specified quiescence}}{{\bf }}
}
\UnaryInfC{
\stackanchor{$\big(
      ec
, \delta!
, \phi^{\delta}_\spec
, \emptyset
, id_{\widehat{A}}
, \emph{INC}^{dur}\big) \in \widehat{Tr}
$}
{
% $
%     \phi^{\delta}_\spec = f^{dur}(ec) \geq \emph{TM}
%     \land \bigvee_{\substack{pec(ec')=ec 
%         \\ chan(ec') \in C^{out} \cup UC^{in} \cup \{\delta\}}} \exists F^{ini}.\pi(ec')
% $
}}
\end{scprooftree}
\end{minipage}
\begin{minipage}{0.45\linewidth}%{9cm}
\centering
\begin{scprooftree}{.76}
\AxiomC{\stackanchor{$ec \in \mathbb{EC}(tp)$}{}}
\LeftLabel{ 
$\begin{array}{r}(R10) \\ \emph{FAIL}^{dur}\end{array}$
%\stackanchor{{\bf R9 Unspecified quiescence}}{{\bf }}
}
\UnaryInfC{
\stackanchor{$\big(
      ec , \delta!%\emph{TM}
, \phi^\delta_\unspec
, \emptyset
, id_{\widehat{A}} 
, \emph{FAIL}^{dur}\big)
    \in \widehat{Tr}
$}
{
% $\phi^{\delta}_\unspec = f^{dur}(ec) \geq \emph{TM}
%     \land \bigwedge_{\substack{pec(ec')=ec 
%         \\ chan(ec') \in C^{out} \cup UC^{in} \cup \{\delta\}}} \forall F^{ini}.\neg \pi(ec')
% $
}}
\end{scprooftree}
\end{minipage}

% \begin{minipage}{11cm}
% \centering
% \begin{scprooftree}{.76}
% \AxiomC{\stackanchor{$ec \in \mathbb{EC}(tp)$}{}}
% \LeftLabel{ (R10) $\emph{FAIL}^{dur}$
% %\stackanchor{{\bf R9 Unspecified quiescence}}{{\bf }}
% }
% \UnaryInfC{
% \stackanchor{
% $\big(
%       ec
% , \delta!%\emph{TM}
% , \phi^\delta_\unspec
% , \emptyset
% , id_{A_{\emph{TC}}}
% , \emph{FAIL}^{dur}
% \big) \in Tr_{\tc}$}{
% \stackanchor{
%  $\phi^\delta_\unspec= f^{dur}(ec) \geq \emph{TM} \land
% \psi^\obs_\unspec$}
% {\stackanchor
% {$ \psi^\obs_\unspec=
%     \bigwedge{\substack{pec(ec')=ec \\ chan(ec') \in C^{out}}} \forall F^{ini}.\forall f^{out}_{chan(ec')}.\neg\pi(ec')
% $}
% {$ \land \bigwedge_{\substack{pec(ec')=ec \\ chan(ec') \in UC^{in}}} \forall F^{ini}. \forall f^{in}_{chan(ec')} . \neg \pi(ec')
% $}
% }
% }}
% \end{scprooftree}
% \end{minipage}
}
%\commental{La symétrie requise par mon biais cognitif ! :-)} \commentbb{Done + correction!}

% $\begin{array}{rllll}
%     \psi^\obs_\unspec =
%     &
%     \bigwedge{\substack{pec(ec')=ec \\ chan(ec') \in C^{out}}}
%     &
%     \forall F^{ini} .
%     &
%     \forall f^{out}_{chan(ec')} .
%     &
%     \neg\pi(ec')
% \\
%     \land
%     &
%     \bigwedge_{\substack{pec(ec')=ec \\ chan(ec') \in UC^{in}}}
%     &
%     \forall F^{ini}.
%     &
%     \forall f^{in}_{chan(ec')} .
%     &
%     \neg \pi(ec')
% \end{array}$

\end{definition}

%Generally speaking, 
A verdict $\text{PASS}$ is reached when $tp$ is covered, verdicts $\text{INC}^m_n$ are reached when traces deviate from $tp$ while remaining in $\mathbb{G}$, and verdicts $\text{FAIL}^m$ denote traces outside $\mathbb{G}$. The annotations $n$ and $m$ provide additional information on the cause of the verdict. Rules $R1$, $R2$ and $R6$, grouped together under the label $\text{SKIP}$, allow advancing along $tp$, resp. by stimulating $LUT$ with the sending of data, observing an emission on $C^{out}$ and observing a reception on $UC^{in}$. Rule $R3$ %(with the label $\text{PASS}$) 
indicates that the last EC of $tp$, thus the $\text{PASS}$ verdict, has been reached. Rules $R4$, $R7$, $R8$ and $R9$, each with a label $\text{INC}^m_n$ indicate that the %last
observed event causes $LUT$ to leave $tp$, without leaving $\mathbb{G}$, resp. by observing an output, an input specified in $\mathbb{G}$, an input not specified in $\mathbb{G}$ and a time-out observation. Lastly, rules $R5$ and $R10$, resp. labeled by  $\text{FAIL}^{out}$ and $\text{FAIL}^{dur}$, raise a $\text{FAIL}$ verdict, for resp. an unauthorized output and an exceeded time-out.
% A verdict $\text{PASS}$ is reached when $tp$ is covered, verdicts of the form $\text{INC}^m_n$ are reached when traces deviate from $tp$ while remaining in $\mathbb{G}$ and verdicts of the form $\text{FAIL}^m$ stand for traces outside $\mathbb{G}$. The annotations $n$ and $m$ provide additional information on the cause of the verdict. 
% Rules $R1$, $R2$ and $R6$, grouped together under the label $\text{SKIP}$, allow advancing along $tp$, resp. by stimulating $LUT$ with the sending of data, observing an emission on $C^{out}$ and observing a reception on $UC^{in}$. Rule $R3$ (with the label $\text{PASS}$) indicates that the last EC of $tp$, thus the $\text{PASS}$ verdict, has been reached. Rules $R4$, $R7$, $R8$ and $R9$, each with a label of the form $\text{INC}^m_n$ indicate that the last observed event causes $LUT$ to leave $tp$, without however leaving $\mathbb{G}$, resp. by observing an output, an input specified in $\mathbb{G}$, an input not specified in $\mathbb{G}$ and a time-out observation. Lastly, rules $R5$ and $R10$, resp. labelled by  $\text{FAIL}^{out}$ and $\text{FAIL}^{dur}$, raise a $\text{FAIL}$ verdict, for resp. an unauthorized output and an exceeded time-out.

%We will comment more in details on the different rules and verdicts using Ex.~\ref{ex:test-case}. %Execution contexts of $tp$ become states of the test case except $tgt(tp)$ which is replaced by $\text{PASS}$. Every verdict state is connected to one or more contexts of $tp$:  Specified output, e.g., transition from $ec_2$ to $\text{INC}^{out}$ inferred from $ec_{10}$, specified uncontrollable input, e.g., transition from $ec_1$ to $\text{INC}^\uncIn_\spec$ inferred from $ec_9$, underspecified uncontrollable input ($\text{INC}^\uncIn_\unspec$), unspecified output ($\text{FAIL}^{out}$), and unspecified quiescence ($\text{FAIL}^{dur}$).



\begin{example}
\label{ex:test-case} In Fig.~\ref{fig:test_case_ATM}, the test case for $tp=ec_0ec_1\ldots ec_4$ (see Ex.~\ref{ex:tiosts-determ}) is depicted. Certain verdict states are repeated for readability, and defining rules annotate the transitions. The test case utilizes the $\text{Transc}$ channel as a controllable input channel for stimulation while observing all other channels. For space considerations, we comment only on some rules.

 \noindent Rule $R1$ defines a stimulation action $\actOut{Transc}(\f{amt_1},\f{\vartime_1})$ (transition from $ec_0$ to $ec_1$) constrained by $\pi(tp)$ to select an appropriate value for $\f{amt_1}$ and $\f{\vartime_1}$ together with a time of stimulation $\f{z_0}$ that allows to remain within the test purpose. E.g., within $\pi(tp)$, $\f{amt_1}$ is limited to some range ($10\leq \f{amt_1} \leq 500$), while $\f{z_0}$ remains unconstrained (a duration measured with clock $\f{z_0}$). All non-revealed variables, i.e., other than $\f{z_0}$, $\f{amt_1}$ and $\f{\vartime_1}$ appearing in $\pi(tp)$ are bound by the existential quantifier due to their unknown values at this execution point. Finally, the clock $\f{z_1}$ is reset to enable reasoning on subsequent actions' duration (measured on $\f{z_1}$). Rule $R2$ defines an observation action $\actIn{Debit}(\f{\freshOut{1}{D}{1}},\f{\freshOut{1}{D}{2}},\f{\freshOut{1}{D}{3}})$  constrained by 
$(\f{z_1}\!<\!\maxWaitingBound) 
\wedge \exists \f{fee_0} . \piAlias{2}$ (transition from $ec_1$ to $ec_2$) while rule $R5$ defines the same observation constrained by 
 $(\f{z_1}\!<\!\maxWaitingBound)
    \land \forall \f{fee_0} .
    \neg \, \piAlias{2}
    \land \forall \{ \f{fee_0} \} \, . \,
    \neg \, \piAlias{9}
    $ (transition from $ec_1$ to $\text{FAIL}^{out}$). Both situations are possible: Trace $(0,\actOut{Transc}(50,4)).
    (0,\actIn{Debit}(1,51,\ATMID))$ reaches $ec_2$ whereas $\text{FAIL}_{out}$ is reached by traces $(0,\actOut{Transc}(50,4)).
    (0,\actIn{Debit}(1,0,\ATMID))$ and $(0,\actOut{Transc}(50,4)).
    (2,\actIn{Debit}(1,51,\ATMID))$ due resp. to data and time non-compliance. Rule $R6$ defines an unspecified quiescence $\delta!$ constrained by $(\f{z_1} \geq \maxWaitingBound)
    \land %\big(
    \forall \f{fee_0} \, . \neg \piAlias{2}
    \land
    \forall \f{fee_0} \, . \neg \piAlias{9}
    \land
    \forall \f{fee_0} \, .\neg \piAlias{10}
    % \big)
$ (transition from $ec_1$ to $\text{FAIL}^{dur}$). The trace $(0,\actOut{Transc}(50,4)).(5,\delta!)$ reaches $\text{FAIL}^{dur}$ (time-out $\maxWaitingBound$ is set to $5$): the time-out is exceeded without the mandatory output on the channel $\text{Debit}$ being observed. Rule $R9$ defines a specified quiescence $\delta!$ (transition from $ec_1$ to $\text{INC}^{dur}$ not drawn for space). This case arises when there is still sufficient time to reach $ec_2$, $ec_9$ or $ec_{10}$ (no quiescence applies from $ec_1$, see Ex.~\ref{ex:quiescence}).
\end{example}
\vspace{-.275cm}

\begin{figure}[t] %[h!]
\vspace{-.275cm}
    \centering
    %\makebox[.9\textwidth][c]{
    
    \resizebox{1\textwidth}{!}{
        \hspace{-1cm}\input{fig/tikz_atm_testcase_simplif}
    }
	\caption{Test case for $\text{ATM}$}
% Tentative version simplifiée pour la lisibilité.
	\label{fig:test_case_ATM}
 \vspace{-.6cm}
\end{figure}

A test case  $\mathbb{TC}$ interacts with a $LUT$, designed to comply with a TIOSTS $\mathbb{G}$, to issue a verdict about a test purpose $tp$. $\mathbb{TC}$ is therefore defined as a mirror image of $\mathbb{G}$: emissions (receptions) in $\mathbb{TC}$ correspond to receptions (emissions) of $\mathbb{G}$ (cf. rules $R1$ and $R2$), except uncontrollable channels whose actions are not reversed (cf rule $R6$). Given a concrete action $act$ (with $v$ for value received or sent), we denote $\overline{act}$ its mirror action, defined as follows: $\overline{c!v} = c?v$ for $c \in C^{out}$, $\overline{c?v} = c!v$ for $c \in CC^{in}$ and  $\overline{c?v} = c?v$ for $c \in UC^{in}$.
We introduce an execution relation that abstracts a synchronized execution of a trace with $\mathbb{TC}$: 
\begin{definition}[Relation execution $\leadsto_{\mathbb{TC}}$]
\label{def:relation-exec}
Let $\mathbb{G}$ be a TIOSTS and $tp$ a test purpose for $\mathbb{G}$ with $\mathbb{TC} = (\widehat{Q},\widehat{q_0},\widehat{Tr})$ the test case guided by $tp$.

The \emph{execution relation}  $\leadsto_{\mathbb{TC}}\subseteq \big( Evt(C_\delta)^* \times  \widehat{Q} \times M^F \big)^2$  is defined by:

for $ev.\sigma \in Evt(C_\delta)^*$, $q,q' \in \widehat{Q}$ and for $\nu, \nu' \in M^F$, $(ev.\sigma,q,\nu) ~\leadsto_{\mathbb{TC}}~ (\sigma, q',\nu')$ holds iff there exists $tr\in \widehat{Tr}$ s.t. $src(tr)\!=\! q$, $tgt(tr)\!=\!q'$, $\nu'(act(tr))=\overline{act(ev)}$ and $M \models_{\nu'} \phi(tr)$ with $\nu'$ defined as:
 \begin{itemize}
     \item if $ev\!=\!(d,c?v)$ and $chan(tr)\!=\!c$ then $\nu'\!=\!\nu[f^{dur}(q)\!\mapsto\!d][ f^{in}_c(q)\!\mapsto\!v]$ ;
     \item if $ev\!=\!(d,c!v)$ and $chan(tr)\!=\!c$ then $\nu'\!=\!\nu[f^{dur}(q)\!\mapsto\!d][f^{out}_c(q) \!\mapsto\! v]$ ;
     \item else, i.e., $ev\!=\!(d,\delta!)$ and $chan(tr)\!=\!\delta$, $\nu'=\nu[f^{dur}(q)\!\mapsto\!d]$.
 \end{itemize}
 \end{definition}


%Let $LUT$ a subset of $ Evt(C_\delta)^*$ satisfying ${\cal H}$. 
%We introduce an execution relation that abstracts a synchronized execution of a $LUT$, given as a subset of $Evt(C_\delta)^*$ satisfying ${\cal H}$, and the test case $\mathbb{TC}$: 
%\vspace{-.275cm}
%\[\leadsto_{\mathbb{TC}}\subseteq \big( Evt(C_\delta)^* \times  \widehat{Q} \times M^F \big)^2  \] 
%\vspace{-.575cm}

Intuitively, a step $(ev.\sigma, q,\nu) ~\leadsto_{\mathbb{TC}}~ (\sigma, q',\nu')$ consists in:
\begin{itemize}
    \item reading the first element $ev$ of a trace from a test case state $q$ and an interpretation $\nu$  synthesizing the known information about the variables in~$F$;
    \item finding a transition $tr$ in $\widehat{Tr}$ whose action matches the mirror action of $ev$; 
    \item building a new triple with $\sigma$ the trace remaining to be read, $q'$ a successor state of $q$ in $\widehat{Q}$, and $\nu'$ the updated interpretation of the variables~$F$. 
\end{itemize}
The execution relation simulates a parallel composition between timed input output systems, synchronizing inputs and outputs. Our formulation deviates from the one in \cite{KrichenT06} for two essential reasons: the symbolic nature of the test case requires the intermediate interpretations of variables to be memorized, and uncontrollable channels require to adapt the synchronization~\cite{EscobedoGGC10}.
Let $LUT$ be a subset of $ Evt(C_\delta)^*$ satisfying ${\cal H}$ and $\overset{*}{\leadsto}_{\mathbb{TC}}$ be the reflexive and transitive closure of  $\leadsto_{\mathbb{TC}}$. Given a $LUT$ trace $\sigma_0$, we apply the execution relation iteratively from an initial triplet consisting of $\sigma_0$ a trace, $ec_0$ an initial EC and $\nu_0$ an arbitrary interpretation, to obtain the corresponding test verdict for $tp$, so that the verdict set obtained from the execution of $\mathbb{TC}$ on $LUT$ is defined by: 

%\noindent $vdt(LUT,\mathbb{TC})= \bigcup_{\substack{\sigma_0\in LUT ,\; \nu_0 \in M^F \\ \text{V}\in\mathbb{V}}}\{\text{V} ~|~ (\sigma_0,{q_0}_{\tc}, \nu_0) \overset{*}{\leadsto}_{\mathbb{TC}} (\sigma,\text{V}, \nu )\}$. 

\noindent $vdt(LUT,\mathbb{TC})= \{\text{V} ~|~ \exists \sigma_0 \in LUT, \nu_0 \in M^F, (\sigma_0,{q_0}_{\tc}, \nu_0) ~\overset{*}{\leadsto}_{\mathbb{TC}} (\sigma,\text{V}, \nu )\}$. 


\noindent Th.~\ref{th:corr} states the soundness of the test case execution for detecting errors through the $\text{FAIL}^{out}$ and $\text{FAIL}^{dur}$ verdicts.  A proof can be found in in Appendix~\ref{anx:proof}. Comparable results can be formulated for the other verdicts. Still, those relating to FAIL verdicts are the only ones to guarantee that any discarded program does not satisfy the tioco conformance relation.

\begin{theorem}
\label{th:corr} 
Let $C$ be a set of channels. Let $\mathbb{G}$ and $LUT$ be resp. a TIOSTS defined on $C$ and a subset of $Evt(C_\delta)^*$ satisfying $\cal{H}$. \\
 If $LUT~tioco~\mathbb{G}$ then for any test purpose $tp$ for $\mathbb{G}$ with $\mathbb{TC}$ as test case guided by $tp$, we have $\emph{FAIL}^{out}\not\in vdt(LUT, \mathbb{TC}) $ and $\emph{FAIL}^{dur}\not\in vdt(LUT, \mathbb{TC})$.
\end{theorem}




%Our test cases can be executed by designing a test program that maintains the following elements: (1) a current state of the test case, some execution context $ec$ (unique by trace-determinism), which is updated by following a test case transition $tr$ corresponding to applied stimulations or processed observations, and (2) a current interpretation $\nu$ that is significant for the revealed variables so-far (from the set $\overline{f}(ec)$). The interpretation $\nu$ is used to evaluate transition guards (whether $M \models_\nu \phi(tr)$) to determine the stimulation's value and the time to send the value or to check observation's value and occurrence time. The test program terminates when a verdict state of the test case is reached. 

%{\em Implementation issues.} 
The test case generation is implemented as module in the Diversity symbolic execution platform~\cite{diversity}. Resulting test cases are expressed in Diversity's entry language, allowing their exploration through symbolic execution with the SMT-solver Z3~\cite{Z3}. For easier execution, we export the test cases from Diversity in JSON format, with transition guards expressed in the SMT-LIB input format for SMT-solvers. Our experiments involved applying this test case generation to the ATM example on an Intel Core i7 processor. Varying the size of the test purposes up to $100$ transitions, we observed successful trace-determinism verification for all test purposes. We noted a noticeable increase in generation duration as the test purpose size grew, while still remaining feasible. Generating the TIOSTS test case ($513$ transitions) for the test purpose of $100$ transitions took more than $40$s, in contrast to only $500$ms for the test purpose of size $4$ in Ex.~\ref{ex:test-case} ($31$ transitions) resp. $8$s for the test purpose of size $50$ ($138$ transitions).



%A simple way of executing our test cases is to design a test program which maintains {\bf{\em (1)}} a current state issued from the test case, i.e., some execution context $ec$ (unique by trace-determinism), which is updated by following some test case transition $tr$ corresponding to a stimulation it applies or an available observation it processes, and {\bf{\em (2)}} a current interpretation $\nu$ significant for the revealed variables so-far, those from the set $\overline{f}(ec)$ that is used to assess transitions' guards (whether $\nu \models \phi(tr)$). The transitions' guards are used to compute stimulations and their submission time (obtained by solving $\phi(tr)$ and remembered through $\nu$) %(proposed by the solver) or to verify observations and their occurrence time (matched through $\nu$ that is checked to satisfy $\phi(tr)$). The test program terminates whenever a verdict state of the test case is reached. We have implemented our test case generation as a module of the symbolic execution platform Diversity~\cite{diversity}.
%A generated test case is expressed in Diversity's entry language as for the reference TIOSTS which allows its exploration by symbolic execution coupled with SMT-solver Z3~\cite{Z3}, e.g., to check the reachability of divergent transitions. We reduce (minimize) the test case to only those reachable transitions. To ease test cases execution, we have exported them from Diversity in the JSON format where test case transitions' guards are expressed in the input format for SMT-solvers, called SMT-LIB.

%We have implemented our test case generation as a module of the symbolic execution platform Diversity~\cite{diversity}. A generated test case is expressed in Diversity xLIA modeling language as for the reference TIOSTS. The test case can then be animated by symbolic execution in Diversity, e.g., to verify the reachability of divergent transitions. Constraint solving required in symbolic execution is done thanks to the SMT-solver Z3~\cite{}. If some divergent transitions are not reachable, we remove them from the test case and reduce (minimize) it to only those reachable transitions. To ease test execution, we have exported it from Diversity in the JSON format where the test case transitions' guards are expressed in the input format for SMT-solvers, called SMT-LIB.










==> macro/macro_tiosts.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TRANSITION
\newcommand{\reset}[1]{\{ {#1} \}}

\newcommand{\guard}[1]{ [ {#1} ] }

\newcommand{\subst}[1]{ \langle {#1} \rangle}

% $tr_ID : q_src \xrightarrow{ 
%   \text{act}{param}, 
%   \guard{cond}, 
%   \reset{clocks},
%   \subst{assigns}
% } q_tgt$
%                         ID  : SRC  -----------  ACT   GUARD       RESET       SUBST ----> TGT
\newcommand{\trans}[7]{ ${#1} : {#2} \xrightarrow{ {#3}, \guard{#4}, \reset{#5}, \subst{#6} } {#7}$ }


==> tab/tab_related_work.tex <==



	\begin{center}
        \small
        \begin{tabular}{|l|c|c|c|c|c|}
	    \hline
		\makecell[c]{\textbf{ Approach }} & \textbf{Time} & \textbf{Symbolic} & \textbf{Online} & \textbf{Relation} & \textbf{Tool} \\ \hline
		
		\cite{Tretmans96a} 1996, Tretmans & $\times$ & $\times$ & $\times$ & ioco & $\times$ \\ \hline
		
		\cite{DuncanJRZ02} 2002, Duncan et al. & $\times$ & $\checkmark$ & $\checkmark$ & ioco & $\checkmark$ \\ \hline
		
		\cite{KrichenT04} 2004, Krichen et al. & $\checkmark$ & $\times$ & $\times$ & tioco & $\checkmark$ \\ \hline
				
		\cite{BohnenkampB05} 2005, Bohnenkamp et al.  & $\checkmark$ & $\times$ & $\checkmark$ & tioco & $\checkmark$               \\ \hline
				
		\cite{GastonGRT06} 2006, Gaston et al.  & $\times$ & $\checkmark$ & $\checkmark$ & ioco & $\checkmark$   \\ \hline
		
		\cite{AndradeMJM11} 2011, Andrade et al. & $\checkmark$ & $\checkmark$ & $\checkmark$ & tioco & $\times$ \\ \hline
		
		\cite{BannourEGG12} 2012, Bannour et al. & $\checkmark$ & $\checkmark$ & $\times$ & tioco & $\checkmark$ \\ \hline
		
% 		\cite{poncedeleonHL12} 2012, Ponce de León et al. & $\times$ & $\times$ & $\checkmark$ & ioco & $\times$ \\ \hline
		
% 		\cite{DavidLMNR13} 2013, David et al. & $\times$ & $\times$ & $\checkmark$ & tioco & $\times$ \\ \hline
		
		\cite{Chimisliu13} 2013, Chimisliu et al. & $\times$ & $\times$ & $\checkmark$ & ioco & $\times$ \\ \hline
		
% 		\cite{Bhateja14} 2014, 	Bhateja &  &  &  & & $\checkmark$ \\ \hline
		
		\cite{GerholdS16} 2016, Gerhold et al. & $\times$ & $\times$ & $\checkmark$ & pioco & $\checkmark$ \\ \hline
		
		\cite{MarssoMS18} 2018, Marsso et al. & $\times$ & $\times$ & $\checkmark$ & ioco & $\checkmark$ \\ \hline
				
	    \end{tabular}
	
	\end{center}
	
	
	


